FlexKalmanNet: A Modular AI-Enhanced Kalman Filter Framework Applied to Spacecraft Motion Estimation

The estimation of relative motion between spacecraft increasingly relies on feature-matching computer vision, which feeds data into a recursive filtering algorithm. Kalman filters, although efficient in noise compensation, demand extensive tuning of system and noise models. This paper introduces FlexKalmanNet, a novel modular framework that bridges this gap by integrating a deep fully connected neural network with Kalman filter-based motion estimation algorithms. FlexKalmanNet's core innovation is its ability to learn any Kalman filter parameter directly from measurement data, coupled with the flexibility to utilize various Kalman filter variants. This is achieved through a notable design decision to outsource the sequential computation from the neural network to the Kalman filter variant, enabling a purely feedforward neural network architecture. This architecture, proficient at handling complex, nonlinear features without the dependency on recurrent network modules, captures global data patterns more effectively. Empirical evaluation using data from NASA's Astrobee simulation environment focuses on learning unknown parameters of an Extended Kalman filter for spacecraft pose and twist estimation. The results demonstrate FlexKalmanNet's rapid training convergence, high accuracy, and superior performance against manually tuned Extended Kalman filters.

==> literature/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> text/XX_materials_and_methods.tex <==
\chapter{Materials and Methods}\label{ch:materials_and_methods}
In this work, an \gls{ai}-based motion estimation algorithm for the state of a tumbling Astrobee is implemented, that expects discrete pose data with additive Gaussian noise and/or structural errors of the Astrobee as measurement input. The output must be the state of the tumbling Astrobee including at least its pose and its twist. Acceleration terms are assumed to be zero which excludes the necessity of inertia parameter estimation \cite{bhat2002computing} and implies constant velocities in the body frame of the target. Since the rotational motion is more challenging to estimate than the translational motion, the estimation of the rotational motion is in bigger focus of this work.

The computational complexity and ease of implementation must be considered when deciding for an appropriate approach, since the algorithm should be capable to run online in a \gls{gnc} pipeline for an Astrobee free-flyer. Therefore, low computation times when using limited hardware like embedded systems are mandatory. In addition, for the \gls{gnc} pipeline, it is required to implement the final estimation algorithm as a standalone \gls{ros} package and providing the estimated state of the Astrobee using the dual quaternion representation. Furthermore, the algorithm should possess certain robustness to be able to handle uncertainties.

In the following, the selected approach, the implementation schemes, the data generation for the to be trained network and the according training scenarios with hyperparameter search are presented. Finally, the evaluation schemes for the selected algorithm are described.


\section{Selected Approach}
Due to the computational intensity of \glspl{ls} and \glspl{pf} algorithms, only \glspl{kf} algorithms are regarded as estimation algorithms for the scope of this work. Within the domain of \glspl{kf}, the \gls{ekf} and the \gls{ukf} are suitable approaches as they are capable to handle non-linearities. The \gls{ukf} offers more flexibility and the potential of more accurate estimations, but requires thereby an optimal tuning for more parameters and additional computational resources than the \gls{ekf}. Therefore, the \gls{ekf} is selected as state estimation algorithm for this work.

Filtering the state-of-the-art approaches presented in \autoref{ch:state_of_the_art} by the decision of using an \gls{ekf}-based approach that applies \gls{ai}, only the EKFNet and the KalmanNet fulfill all requirements mentioned at the beginning of this chapter. Both approaches apply \glspl{rnn} to learn constant unknown parameters of the \gls{kf}. Since KalmanNet is replacing partial dynamics required for non-linear systems with its \gls{rnn}-based core, and the dynamics of the system (except the noise covariances) of this work are fully known, using the known dynamics is more promising and requires less intensive training of a model. Hence, EKFNet, that focuses solely on learning the noise covariances is the best-fitting approach for this work.

However, since computational restrictions are system-dependent and changing over time, which may allow to use a \gls{ukf} instead of an \gls{ekf} in the future, and none of the approaches in the literature allows to use both an \gls{ekf} and a \gls{ukf}, a novel and modular approach is selected and presented in this work. This novel approach enables to use different variants of \glspl{kf} while fulfilling the requirements of this thesis and making a scientific contribution by filling a research gap. It provides a framework to train a \gls{dfcnn} to learn unknown parameters of a \gls{kf} from measurement data whereby the \gls{kf} is treated modularly and thus can be substituted with any variant of \glspl{kf}. Hence, the parameters to be learned can be chosen with full flexibility. Due to the usage of an \gls{ann} architecture, and the modular flexibility for applying different \gls{kf} variants and learning any parameters of interest, this proposed framework is named FlexKalmanNet. FlexKalmanNet augments the existing state-of-the-art approaches by providing a generalized framework.

Unlike KalmanNet and EKFNet, the training of FlexKalmanNet does not rely on the sequential nature of data and the learning restrictions associated with it, since the sequential computation of the data is outsourced to the \gls{kf} variant. This allows the use of a \gls{dfcnn} model that is - compared to \glspl{rnn} (which are applied to integrate the sequential nature of the data in KalmanNet and EKFNet) - advantageous for efficient large data handling and complex feature extraction, relevant for successful learning \cite{alom2019state}. Furthermore, \glspl{rnn} focus on local contexts whereas \glspl{fnn} can capture global patterns due to their ability to connect any input to any output which makes the approach of FlexKalmanNet very promising.

As a result of the inclusion of a modular \gls{kf} instance in the training, the learning of FlexKalmanNet is a chained process instead of an end-to-end process. It learns by forwarding a set of measurements through the network, which outputs the parameters to be learned. The selection of the to be learned parameters thereby depends on the specific scenario and the selected \gls{kf} variant. Both, the set of measurements and the model's output (the learned parameters) are then passed to the \gls{kf} instance, which outputs a set of estimated states. This set of estimated states is eventually used to compute the loss with the available (partial) data from the true states.

For the purpose of this work, an \gls{ekf} is placed in the FlexKalmanNet with the aim of learning the unknown noise covariances, i.e. the process noise covariance matrix $\boldsymbol{Q}$ and the measurement noise covariance matrix $\boldsymbol{R}$. A simplified computational graph of the forward pass of FlexKalmanNet is depicted in \autoref{fig:computational_graph}, which also shows how the noisy measurements are used for both the \gls{dfcnn} (globally) and the \gls{kf} variant (sequentially).

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/computational_graph.pdf}
\caption[Forward pass of the computational graph of FlexKalmanNet]{\textbf{Forward pass of the computational graph of FlexKalmanNet.} The flow of activations during a forward pass is illustrated via the solid arrows. The dashed arrows represent data flows that are relevant for the framework, but not part of the computational graph. The backward pass for the gradients goes in the opposite direction of the illustrated solid lines.}
\label{fig:computational_graph}
\end{figure}

Due to the sequential nature of the \gls{kf}, the flow of the computational graph of FlexKalmanNet reveals a sequential behavior that is comparable to \gls{bptt} \cite{gruslys2016memory}, the backpropagation that is required for \glspl{rnn}.


\section{Data Generation}\label{sec:data_generation}
Two sources are utilized in this work to generate data, a Python framework and the \gls{ros}-based \gls{ars}. The data from the Python framework is used for principal testings of the \gls{ekf} implementation. It provides a simple sequence of orientations as quaternions in the world frame and the corresponding angular velocities in the world frame, generated based on given angular velocities in the body frame and a defined length of the sequence. Similarly, positions can be generated. The data is exported as \gls{csv} file to ensure full compatibility for any use. Additive Gaussian noise can be applied to the quaternions and positions from the data to simulated noisy measurements.

For training and evaluation, the data from the other source, the \gls{ars}, is applied, trying to make use of the data closest to real-scenario data. Therefore, in the simulation environment, an Astrobee can be set to rotate at a defined position with set angular velocities in the body frame. The \gls{ars} rotation simulations include more dynamics of the physical world, making the data more realistic. Recording the data as rosbag and exporting it to a \gls{csv} makes this data usable for \gls{ros}-independent applications. Two rosbags with the following angular velocities are recorded:

\begin{itemize}
    \item \textbf{\gls{ds1}}, Realistic velocity: $\boldsymbol\omega = [0.02, 0.04, 0.06]$, which is about double of the magnitude of rotation of the in Earth's orbit tumbling satellite Envisat \cite{silha2016comparison}.
    \item \textbf{\gls{ds2}}, Excessive velocity: $\boldsymbol\omega = [0.1, 0.2, 0.3]$, which is used to analyse stability and sensitivity of the trained \gls{ekf}.
\end{itemize}

Since the challenge of this work is prioritizing to estimate the rotational motion right, the translational velocity is set to 0 for the data recordings. Both of the rosbags are recorded with a rate of 10 \gls{hz} and provide 16000 samples each.

In the measurement data, the unit quaternions data does not require a normalization as data preprocessing step, since unit quaternion values are already guaranteed to be between -1 and 1. The position data, in turn, mostly is on another scale than unit quaternions, which is why the position data should be normalized before training to ensure that all input features are in comparable scales for better convergence during training \cite{huang2023normalization}. Therefore, different types of normalization can be applied, where \textit{min-max feature scaling} and \textit{standard score} are very common approaches \cite{patro2015normalization}. For the positions, standard score normalization is applied, which allows for outliers, which are statistically given by the additive Gaussian noise.

The applied Gaussian noise has a standard deviation $\sigma = 0.1$ and a mean $\mu = 0$. For positions, this noise is simply added to the measurements. For the quaternions, in turn, the noise is applied as an error rotation quaternion which is built using the standard deviation as rotation angle for each axis in rad. This yields a probabilistic rotation error magnitude of around $10\hspace{0.1pt}^{\circ}$, which is assumed to be sufficient as simulated large noise in the orientation data.


\section{Implementation Schemes}\label{sec:implementation_schemes}
In this section, simplified pseudo codes are presented to sketch the implementations of this work. The algorithms are implemented in Python using the \gls{ml} library \textit{PyTorch}, and \CC\hspace{0pt} using the linear algebra library \textit{Eigen}. Python is used for the implementation of FlexKalmanNet since for Python more libraries for \gls{ml} are available. The \gls{ros} package with the online \gls{ekf}, in turn, is implemented in \CC\hspace{0pt} to provide better computation times. Since for both, the FlexKalmanNet and the \gls{ros} package, an \gls{ekf} implementation is required, the \gls{ekf} is implemented in Python and \CC\hspace{0pt}. All implementations with instructions for configuration and execution, and the generated and utilized data will be available on GitHub\footnote{
Repository of \glspl{ekf}: \url{https://github.com/MoritzDPTV/ekf_quaternions}\\
\mbox{}\hspace{18pt}Repository of FlexKalmanNet: \url{https://github.com/MoritzDPTV/FlexKalmanNet}\\
\mbox{}\hspace{18pt}Repository of the \gls{ros} package: \url{https://github.com/MoritzDPTV/ekf_ros_package}} following a possible publication in a scientific journal.


\subsection{Extended Kalman Filter Implementation}
In this section, both implementations for the offline and online \gls{ekf} are presented. \autoref{alg:ekf_offline} depicts the implementation of the \gls{ekf} for offline purposes such as learning or testing.

\begin{algorithm}[!ht]
\begin{algorithmic}[1]
\vspace{5pt}
\Function{\textsc{runEKF}}{$dt, correction\_step, measurements, \sigma\_q, \sigma\_r$}\vspace{3pt}
\State \textsc{initEKF}()\vspace{3pt}
\For {$i$ in range of $0..length\_measurements$}\vspace{3pt}
\State \textsc{ekfPredict}($dt, \sigma\_q$)\vspace{3pt}
\If {$i$ modulo $correction\_step$ is $0$}\vspace{3pt}
\State \textsc{ekfCorrect}($measurement[i], \sigma\_r$)\vspace{3pt}
\State \textsc{appendStateToList}()\vspace{0pt}
\EndIf
\EndFor
\State \Return $list\_states$\vspace{5pt}
\EndFunction
\end{algorithmic}
\caption[Extended Kalman filter - offline]{\hspace{-4pt}\textbf{: Extended Kalman filter - offline}}
\label{alg:ekf_offline}
\end{algorithm}\vspace{6pt}

The \textsc{initEKF} function sets the initial global variables such as first estimates of the state and the error state covariance, and initializes an empty list to collect the states. The functions \textsc{ekfPredict} and \textsc{ekfCorrect} compute the new state and the new error state covariance using \autoref{eq:ekf_prediction_1} to \autoref{eq:ekf_correction_5} and the motion dynamic models of interest. \textsc{ekfCorrect} is thereby only called every $n^{th}$ time to simulate the lack of measurement data, where $n$ is defined by the variable $correction\_step$. Thereby, many measurements are skipped, but a ground truth within the data exists for all applied predictions. For scenarios of limited data, the ground truth can be interpolated to make use of every single measurement even when simulating a lack of data. After every \gls{ekf} correction, the new estimated and corrected state is appended to a list of states, that is returned after all measurements are processed and can be used for plotting and further analysis.

In \autoref{alg:ekf_online} the online version of the \gls{ekf} applied in the \gls{ros} package is presented.

\begin{algorithm}[!ht]
\begin{algorithmic}[1]
\vspace{5pt}
\Function{\textsc{runNode}()}{}\vspace{3pt}
\State \textsc{initEKF}()\vspace{3pt}
\State \textsc{initTimer}()\vspace{3pt}
\State \textsc{initSubscriber}()\vspace{3pt}
\State \textsc{initPublisher}()\vspace{3pt}
\EndFunction
\Function{\textsc{getMeasurement}()}{}\vspace{3pt}
\State \textsc{setNewMeasurement}()\vspace{3pt}
\EndFunction
\Function{\textsc{runEKF}}{$dt, \sigma\_q, \sigma\_r$}\vspace{3pt}
\State \textsc{ekfPredict}($dt, \sigma\_q$)\vspace{3pt}
\If {$new\_measurement$ is available}\vspace{3pt}
\State \textsc{ekfCorrect}($new\_measurement, \sigma\_r$)\vspace{3pt}
\State \textsc{constructDualQuaternion}()\vspace{3pt}
\State \textsc{publishToTopic}()\vspace{5pt}
\EndIf
\EndFunction
\end{algorithmic}
\caption[Extended Kalman filter - online]{\hspace{-4pt}\textbf{: Extended Kalman filter - online}}
\label{alg:ekf_online}
\end{algorithm}\vspace{6pt}

In the online implementation of the \gls{ekf}, a node is implemented that handles the selective execution of the \gls{ekf} prediction and correction. The node is started calling \textsc{runNode}, which initializes the \gls{ekf}, a timer to run the \gls{ekf} via \textsc{runEKF} of the online version with a defined frequency, and a subscriber and publisher to listen to the topic containing the measurements and to register a new topic to post the resulting \gls{ekf} states in. The artificial correction step variable is thus left out in this implementation. Instead, an if-statement is checking if a new measurement is available, which is the case, if the function \textsc{getMeasurement} is called by the subscriber on receive of a new message, which is then saved globally. If a new measurement is available, the \gls{ekf} correction is performed yielding the new best state estimate which is then converted to dual quaternions as described in \autoref{eq:dual_quaternion_pose_wf} and \autoref{eq:dual_quaternion_twist_wf}, and eventually published in the new topic. If no new measurement is available, the state is solely propagated via the \gls{ekf} predict function and saved in the variables of the \gls{ekf} instance.\\

The dual quaternion conversion is applied as an additional step instead of using dual quaternion dynamics already in the \gls{ekf} with the following reason: The state processed by the \gls{ekf} consists of quaternions, positions, angular velocities and translational velocities, which sum up to a state vector size of 13. Utilizing a dual quaternion representation as state vector, in turn, requires a state vector with the size of 16. Accordingly, the Jacobian of the state transition model has the size $16 \times 16$ instead of $13 \times 13$, which is an increase of over 66 \% of variables in this single matrix. Hence, the post hoc conversion of the dual quaternions is the computationally more efficient approach and selected therefore.\\


\subsection{FlexKalmanNet Implementation}
For the implementation of FlexKalmanNet, two implementation schemes are presented. First, the run function that starts the training, then the implementation of the \gls{dfcnn}.

\begin{algorithm}[!ht]
\begin{algorithmic}[1]
\vspace{6pt}
\Function{\textsc{RunFlexKalmanNet}}{$config, data$}\vspace{3pt}
\State \textsc{preprocessData}($config, data$)\vspace{3pt}
\State \textsc{initDynamicDFCNN}($config$)\vspace{3pt}
\State \textsc{initLossFunction}($config$)\vspace{3pt}
\State \textsc{initOptimizer}($config$)\vspace{3pt}
\State \textsc{initEKF}($config$)\vspace{3pt}
\For {$epoch$ in range 0..$num\_epochs$}\vspace{3pt}
\For {$batch\_train$ in $data\_train$}\vspace{3pt}
\State \textsc{resetOptimizerGradients}()\vspace{3pt}
\State $\sigma\_q\_train, \sigma\_r\_train \gets$ \textsc{DynamicDFCNN}($batch\_train$)\vspace{3pt}
\State $ekf\_state\_train \gets$ \textsc{runEKF}($batch\_train, \sigma\_q\_train, \sigma\_r\_train$)\vspace{3pt}
\State $loss\_train \gets$ \textsc{computeLoss}($ekf\_state\_train, batch\_train$)\vspace{3pt}
\State \textsc{computeGradients}($loss\_train$)\vspace{3pt}
\State \textsc{updateParametersWithOpimizedGradients}()\vspace{3pt}
\State \textsc{appendTrainLossToTrainList}($loss\_train$)
\EndFor
\For {$batch\_val$ in $data\_val$}\vspace{3pt}
\State $\sigma\_q\_val, \sigma\_r\_val \gets$ \textsc{DynamicDFCNN}($batch\_val$)\vspace{3pt}
\State $ekf\_state\_val \gets$ \textsc{runEKF}($batch\_val, \sigma\_q\_val, \sigma\_r\_val$)\vspace{3pt}
\State $loss\_val \gets$ \textsc{computeLoss}($ekf\_state\_val, batch\_val$)\vspace{3pt}
\State \textsc{appendValLossToValList}($loss\_val$)
\EndFor
\State \textsc{saveBestModel}()\vspace{3pt}
\State \textsc{checkEarlyStoppingConditions}()\vspace{3pt}
\State \textsc{adjustLearningRate}()\vspace{3pt}
\If {$show\_progress$ is True}\vspace{3pt}
\State \textsc{printAndPlotProgress}()
\EndIf
\EndFor
\State \textsc{loadBestModel}()\vspace{3pt}
\For {$batch\_test$ in $data\_test$}\vspace{3pt}
\State $\sigma\_q\_test, \sigma\_r\_test \gets$ \textsc{DynamicDFCNN}($batch\_test$)\vspace{3pt}
\State $ekf\_state\_test \gets$ \textsc{runEKF}($batch\_test, \sigma\_q\_test, \sigma\_r\_test$)\vspace{3pt}
\State $loss\_test \gets$ \textsc{computeLoss}($ekf\_state\_test, batch\_test$)\vspace{3pt}
\State \textsc{appendTestLossToTestList}($loss\_test$)
\EndFor
\State \textsc{saveConfigAndBestSigmas}()\vspace{3pt}
\If {$perform\_full\_run$ is True}\vspace{3pt}
\State \textsc{runEKFOnAllDataWithBestSigmasAndPlotResults}()\vspace{5pt}
\EndIf
\EndFunction
\end{algorithmic}
\caption[FlexKalmanNet - run]{\hspace{-4pt}\textbf{: FlexKalmanNet - run}}
\label{alg:fkn_run}
\end{algorithm}

The scheme of the implementation of the FlexKalmanNet run function is presented in \autoref{alg:fkn_run}. The principle phases for a training, presented in \autoref{sec:ann}, are required when implementing an \gls{ann} and thus also part of the FlexKalmanNet implementation. After the data preprocessing, that includes the standardization of non-quaternion data, the \gls{dfcnn}, the loss function, the optimizer and the \gls{ekf} are initialized based on the given config file and data. The selection of hyperparameters in the config file is presented in the subsequent section (\autoref{sec:trainaing_scenarios}). Since the hyperparameters for the \gls{dfcnn} are allowed to vary, the \gls{dfcnn} is implemented dynamically. After the initializations, throughout the epochs, the training and validation phases are conducted forwarding the input batches through the \gls{dfcnn} saving the best model based on the validation loss. If the validation loss is not decreasing over a in the config defined number of epochs, the training is stopped. Otherwise, the learning rate is adjusted if necessary and the progress is optionally shown. After all epochs, the best model is eventually utilized for the test phase, whereupon the sigmas of the best model, the test and validation loss, and all hyperparameters of the training are saved in a file. An \gls{ekf} run on the full data can optionally be performed at the very end using the best sigmas for evaluation. Furthermore, the \gls{ekf} instance can be replaced by other \gls{kf} instances, which only requires adjustments of the output from the \gls{dfcnn}.

\begin{algorithm}[!ht]
\begin{algorithmic}[1]
\vspace{6pt}
\Class{\textsc{DynamicDFCNN}}{$config$}\vspace{3pt}
\Function{initNetwork}{$config$}\vspace{3pt}
\State \textsc{checkIfInputOutputSizeAreValid}($config$)\vspace{3pt}
\For{$i$ in range 0..$num\_layers - 1$}\vspace{3pt}
\State \textsc{appendLinearLayerToLayerList}($config$)\vspace{3pt}
\State \textsc{appendActivationFunctionToLayerList}()\vspace{3pt}
\State \textsc{appendDropoutToLayerList}($config$)
\EndFor
\State \textsc{appendLinearOutputLayerToLayerList}($config$)\vspace{3pt}
\State \textsc{buildSequentialModelFromLayerList}()\vspace{3pt}
\EndFunction
\Function{forwardData}{$data$}\vspace{3pt}
\State $output\_model \gets$ \textsc{feedDataThroughTheModel}($data$)\vspace{3pt}
\State $output\_model \gets$ \textsc{absoluteOutputs}($output\_model$)\vspace{3pt}
\State $output\_model \gets$ \textsc{meanOutputsToSampleSize}($output\_model$)\vspace{3pt}
\State $output\_model \gets$ \textsc{limitOutputToRange}($output\_model$)\vspace{3pt}
\State \Return $output\_model\_split\_1, output\_model\_split\_2$\vspace{5pt}
\EndFunction
\EndClass
\end{algorithmic}
\caption[FlexKalmanNet - dynamic deep fully connected neural network]{\hspace{-4pt}\textbf{: FlexKalmanNet - dynamic \gls{dfcnn}}}
\label{alg:fkn_dfcnn}
\end{algorithm}

In \autoref{alg:fkn_dfcnn}, the implementation of the \gls{dfcnn} of FlexKalmanNet is shown. In order to find the best fitting hyperparameters, the architecture of the \gls{dfcnn} needs to be dynamic. Therefore, a for-loop is implemented in the initialization function of the model that iterates through the defined number of layers reduced by 1 appending a linear layer, an activation function module and a dropout module to a list with every iteration. After the last iteration, a final output layer is appended. The list of layers and modules is then composed to a sequential model. In the forward function of the model, the data is fed through the network yielding the model's output. The absolute value of this output is then averaged along its column to have a resulting set of output parameters fitting the parameter number required for the \gls{ekf}. Furthermore, to avoid output values outside the range of interest, the output is clipped. Thereby, the maximum terms for the noise covariance are set to be limited to 1, possibly manoeuvring the \gls{ann} to not push further in its current direction. Depending on the desired output size and output variables, the output of the model is then subdivided into the desired format. To ensure, output sizes fit the implemented metrics in the forward function, at the beginning of the initialization function, a validation check for the input size and output size of the passed config is implemented.


\section{Training Scenarios and Hyperparameter Search}\label{sec:trainaing_scenarios}
Training scenarios should simulate scenarios that either are close to real-life scenarios or scenarios for verification purpose such as the proving of robustness of a system. For both cases, data with additive noise is generated as described in \autoref{sec:data_generation}. This data is used to train the \gls{dfcnn} to learn the noise covariances for the measurement noise $\boldsymbol{R}$ and the process noise $\boldsymbol{Q}$ for an \gls{ekf} to run offline filtering data from the same source used for the training data.

In the defined training scenario that fulfills the requirements of this work, the \gls{ekf} has a state vector of the size 13, which includes the pose and its derivative features, the twist. The dynamics of this scenario are derived in \autoref{sec:ekf_state}. The expected measurements in this scenario contain only pose data, i.e. position and orientation (as quaternion) data. These conditions require 7 parameters for the measurement noise covariance matrix $\boldsymbol{R}$ and another 13 parameters for the process noise covariance matrix $\boldsymbol{Q}$, which add up to 20 unknown variables. Hence, the \gls{dfcnn}'s output size must be 20. To match the available measurement feature size for the \gls{ekf} with the input for the \gls{dfcnn}, the input size of the \gls{dfcnn} must be 7. \autoref{tab:training_scenarios} gives an overview about the input and output sizes for the \gls{ekf} and the \gls{dfcnn}.

\begin{table}[!ht]
\centering
\caption[Input and output sizes for the deep fully connected neural network and the extended Kalman filter]{Input and output sizes for the \gls{dfcnn} and the \gls{ekf}}
\begin{tabular}{cccc}
\hline
\hline
\addlinespace
Input \gls{ekf} & Output \gls{ekf} & Input \gls{dfcnn} & Output \gls{dfcnn} \\
\addlinespace
\toprule
\addlinespace
7 & 13 & 7 & 20 \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:training_scenarios}
\end{table}\vspace{10pt}

The loss within the training phase of the \gls{dfcnn} is computed using all estimated state features from the \gls{ekf} for the given noisy measurements, and the noise-free measurements as ground truth. Furthermore, to enhance the learning, a cut for the losses is introduced, that ignores a defined first part of the estimated states and the corresponding ground truths when computing the loss to reduce the impact of large errors during the settling time of the \gls{ekf}. It is also possible to apply a weighting policy to all losses instead, but doing so may introduce a bias to the learning, which is why the cut is chosen as loss optimization \cite{byrd2019effect}.

Besides the loss cut, there are many other hyperparameters, that must be set before starting the training. In \autoref{tab:hyperparameter_large}, a hyperparameter space of heuristically preselected hyperparameters is given, providing an overview about available hyperparameters for FlexKalmanNet.

\begin{table}[!ht]
\centering
\caption[Heuristic hyperparameter space for FlexKalmanNet]{Heuristic hyperparameter space for FlexKalmanNet where for each hyperparameter a set of 1 to 5 values is defined}
\begin{tabular}{l|c}
\hline
\hline
\addlinespace
Hyperparameter & Set of values \\
\addlinespace
\toprule
\addlinespace
Random seed & [0] \\
Input size & [7] \\
Output size & [20] \\
Batch size & [512] \\
Hidden size & [256, 512, 1024, 2048] \\
Number of layers & [4, 5, 6, 7, 8] \\
Learning rate & [$1e^{-6}$, $1e^{-5}$, $1e^{-4}$, $1e^{-3}$] \\
Dropout probability & [0, 0.25, 0.5] \\
Weight decay penalty term & [0, $1e^{-5}$, $1e^{-3}$] \\
Loss function & [\gls{mse}] \\
Loss scheduler & [\gls{relrop}] \\
Loss cut & [100] \\
Optimizer & [\gls{adam}] \\
Activation function & [Leaky\gls{relu}] \\
Number of epochs & [100] \\
Early stopping after epochs & [20] \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:hyperparameter_large}
\end{table}\vspace{10pt}

The \textit{random seed} is a variable the can be set in the utilized random engine before executing random operations such as generating random normal distributed noise or initializing the weights and biases of a model to ensure reproducability. It is selected to be 0 with no other intention than having a fixed value. The batch size is defined as 512 to benefit from the mini-batch advantages, while still maintaining enough length for the \gls{ekf} to converge and maintain the states over some time even when introducing a loss cut of 100 to ignore the settling time for the loss computation. The selected loss function and loss scheduler \gls{mse} and \gls{relrop} are both robust policies, suitable for supervised learning \cite{ghosh2017robust}. The optimizer is selected to be \gls{adam} which is recommended for deep \gls{ann} architectures due to its efficiency and robustness \cite{zhang2018improved}. As the activation function, Leaky\gls{relu} is applied since it introduces non-linearities while avoiding that neurons become too small due to negative gradients keeping all neurons active \cite{xu2020reluplex}. The two last fixed hyperparameters are the number of epochs and the early stopping variables. The number of epoch of 100 is selected based on primary runs exhibiting converging phases already after 20 epochs and less, the early stopping length is accordingly selected to train at least for the observed convergence phase while efficiently allowing to save resources.

Even with most of the hyperparameters being fixed by having a only one option in the preselected hyperparameter space, those five hyperparameters being still variable with 3 to 5 options each extend the space to have $4 \cdot 5 \cdot 4 \cdot 3 \cdot 3 = 720$ possible combinations. To circumvent the necessity of running such an amount of trainings to find well suited hyperparameters, random search methods can be applied. \Gls{wandb}\footnote{Website: \url{https://wandb.ai/}} is an \gls{api} that can be utilized for hyperparameter search, rich visualization and interactive experiment tracking. Hence, running trainings of e.g. 100 randomly selected possible hyperparameter combinations, also called \textit{sweeps}, does not reveal the best combination, but exhibit patterns useful to reduce the hyperparameter space. This can be repeated until a realizable number of combinations is left for which a full grid search can be conducted, as well using \gls{wandb}.

With further heuristic tests, the hyperparameter space is further reduced as presented in \autoref{tab:hyperparameter_grid}. To find the best hyperparameters for both datasets, a grid search is applied to this reduced hyperparameter space. Subject of this search is not only finding best-fitting hyperparameters for each dataset, but also trying to find a hyperparameter set, that fits both datasets and yields the potential of a general solution for other datasets with different angular velocities of similar training scenarios. This reduced hyperparameter space enables with the four left variable hyperparameters $2 \cdot 3 \cdot 2 \cdot 2 = 24$ possible combinations, meaning 24 \gls{wandb} sweeps.

\begin{table}[!ht]
\centering
\caption[Reduced hyperparameter space for a grid search]{Reduced hyperparameter space for a grid search where for each hyperparameter a set of 1 to 3 values is defined}
\begin{tabular}{l|c}
\hline
\hline
\addlinespace
Hyperparameter & Set of values \\
\addlinespace
\toprule
\addlinespace
Random seed & [0] \\
Input size & [7] \\
Output size & [20] \\
Batch size & [512] \\
Hidden size & [512, 1024] \\
Number of layers &  [6, 7, 8] \\
Learning rate & [$1e^{-5}$] \\
Dropout probability & [0, 0.5] \\
Weight decay penalty term & [0, $1e^{-3}$] \\
Loss function & [\gls{mse}] \\
Loss scheduler & [\gls{relrop}] \\
Loss cut & [100] \\
Optimizer & [\gls{adam}] \\
Activation function & [Leaky\gls{relu}] \\
Number of epochs & [100] \\
Early stopping after epochs & [20] \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:hyperparameter_grid}
\end{table}\vspace{10pt}

Since the \gls{ann} training consists of the three phases, training, validation and testing, the utilized data must be split to provide data for each phase. Therefore, the data is divided into proportions of 80\,\% for training, 10\,\% for validation, and 10\,\% for testing.

The training is conducted on a virtual server, equipped with a \gls{ssd} drive, with 8 \gls{gb} of memory, and with 4 virtual cores accessing a \textit{AMD EPYC 7452 Rome} \gls{cpu} providing 32 cores with each 2.35 \gls{ghz} clock speed. The virtual server runs on Ubuntu 20.04 and does not have access to a \gls{gpu}.


\section{Testing and Evaluation Metrics}\label{sec:test_eval_metrics}
In order to test and evaluate the \gls{ekf} using trained parameters, suitable hyperparameters for the \gls{dfcnn} for both datasets must be found to learn the required \gls{ekf} parameters. The decision for a specific set of hyperparameter can be made based on the following criteria:

\begin{itemize}
    \item \textbf{Learned parameter space}: Are there learned parameters that reached the maximum allowed value of 1?
    \item \textbf{Training convergence}: How long does the validation loss take to converge in terms of epochs and time?
    \item \textbf{Model accuracy}: How accurate are the test \gls{ekf} results of the trained model?
\end{itemize}

The \gls{ekf} using the best-found learned parameters is tested offline and online. Offline, the trained \gls{ekf} is run and evaluated on the full recorded datasets from the \gls{ars} and not only on batches as for the training, since an \gls{ekf} run on the short length of a batch may not reveal instability over time. Online, the trained \gls{ekf} is tested using the \gls{ars} to simulate a real-life and real-time scenario as verification for the online functionality and the implemented \gls{ros} package. Since in real-life measurements may be only available in a low frequency, for the testings, lack-of-data mechanisms (see \autoref{sec:implementation_schemes}) are deployed to approve the \gls{ekf} propagation and verify stability in terms of few measurements availability. With the ground truth available in the data and in the \gls{ars}, the \gls{ekf} state estimates can directly be compared to determine its accuracy.

The following list presents the evaluation criteria to test the \gls{ekf}'s functionality using the trained parameters:

\begin{itemize}
    \item \textbf{Accuracy}: How accurate are the state estimates from the \gls{ekf}?
    \item \textbf{Stability}: How stable is the \gls{ekf} over time?
    \item \textbf{Robustness}: How robust is the \gls{ekf} with regard to different noises and different velocities in the data?
    \item \textbf{Sensitivity}: How sensitive is the \gls{ekf} to changes in the data?
    \item \textbf{Settling time}: How long does the \gls{ekf} take to settle?
\end{itemize}

In addition to the offline and online functionality test, the performance of the trained \gls{ekf} is evaluated offline via the following metric:

\begin{itemize}
    \item \textbf{Baseline}: How well does the \gls{ekf} using the trained parameters perform compared to manually tuned parameters?
\end{itemize}

In the baseline \gls{ekf}, for the diagonal entries of the measurement noise covariance matrix $\boldsymbol{R}$, the ground truth standard deviation of the noise $\sigma_R = 0.1$ is applied. Since the dynamics of the quaternions and angular velocities are linearized approximations, the diagonal entries of the process noise covariance matrix $\boldsymbol{Q}$ for the quaternion components and angular velocities is set to $\sigma_{Q_{rot}} = 0.005$. For the positions and translational velocities, perfect model dynamics and thus lower entries for process noise covariance matrix $\boldsymbol{Q}$ can be assumed, wherefore $\sigma_{Q_{trans}} = 0.0001$ is selected.


==> text/XX_results_and_discussion.tex <==
\chapter{Results and Discussion}\label{ch:results_and_discussion}
The presented \gls{ai}-based motion estimation algorithm for a state including the rotational and translational motion is tested and evaluated in this chapter. Therefore, hyperparameter searches using \gls{wandb} and training results of both datasets, \gls{ds1} and \gls{ds2} (see \autoref{sec:data_generation}) are considered. With the best trained parameters of the different datasets, the \gls{ekf} using these learned parameters is then analysed and finally compared to a baseline: a manually tuned \gls{ekf}.

As measurement for the accuracy, the \gls{rmse} is applied to compute the loss of the estimated and the true states. The \gls{rmse} is an extension to the \gls{mse}, applying the square root to the \gls{mse} to yield the original domain of the loss variables.


\section{Training Results}
For the analysis of the hyperparameter search, as a representative example the results of \gls{ds1} are demonstrated. The hyperparameter search results of \gls{ds2} can be found in the \hyperref[appendix_hyper]{Appendix A.1}.

The first aspect to analyse are the learned parameters. If the model tries to compensate noise with high values in the learned noise covariances, those sweeps are excluded, since these solutions are overfitting solutions. \textit{High values} means equal to 1, since higher values are clamped to 1 in the model's output (see \autoref{sec:implementation_schemes}). \autoref{fig:maximum_sigma_value} presents the largest of the learned parameters of every sweep in each epoch.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/maximum_sigma_value.pdf}
\caption[Largest learned covariance parameters during training]{\textbf{Largest learned covariance parameters during training.} This graph depicts the largest of the learned parameters of 24 sweeps, tracked over each epoch during the hyperparameter search for \gls{ds1}. The learned parameters are standard deviation terms.}
\label{fig:maximum_sigma_value}
\end{figure}

Since none of the 24 sweeps exhibit invalid noise compensation with large learned parameter terms, no exclusion of sweeps is necessary. Furthermore, the evolution and convergence of the largest learned parameters already indicates stability within the training. In order to further analyse the sweeps, the accuracy of the sweeps is inspected. Therefore, a graph that maps the sweeps along hyperparameter columns to the validation loss of the best model is utilized (see \autoref{fig:sweeps_ds1_filter_0}).

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/sweeps_ds1_filter_0.pdf}
\caption[Full hyperparameter space mapped to the best validation loss for dataset 1]{\textbf{Full hyperparameter space mapped to the best validation loss for \gls{ds1}.} Each of the columns represent a variable in the hyperparameter space that has more than one value available. The sweeps are traversing these columns from the left hand side to the right hand side, mapping their hyperparameters to their best validation loss as \gls{rmse}. The color map also indicates the magnitude of the loss relative to the minimum and maximum loss values of all sweeps.}
\label{fig:sweeps_ds1_filter_0}
\end{figure}

The first view on \autoref{fig:sweeps_ds1_filter_0} seems to indicate, that using a weight decay of 0 yields higher validation losses. One might assume, that excluding the node of the weight decay of 0 may be a first good filtering move. By looking closer at the graph, it can be seen, that many sweeps using the weight decay of 0 also end up in the lowest loss area of this hyperparameter search. Therefore the impact of other variables is observed, yielding the first filtered operation presented in \autoref{fig:sweeps_ds1_filter_1}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/sweeps_ds1_filter_1.pdf}
\caption[Reduced hyperparameter space mapped to the best validation loss for dataset 1]{\textbf{Reduced hyperparameter space mapped to the best validation loss for \gls{ds1}.} In the column of the dropout probability, at the bottom a filter box is set, allowing only values of the column within the filter box. Thereby, paths of sweeps outside the filter are greyed-out.}
\label{fig:sweeps_ds1_filter_1}
\end{figure}

Filtering for having only sweeps with a dropout probability of 0, removes the runs with the high losses that seemed to be related to the weight decay of 0. This first filtering reduces the runs to be in a fairly similar \gls{rmse} error range. By observing the loss more closely, the hyperparameter space can be further reduced to a final set of hyperparameters as demonstrated in \autoref{fig:sweeps_ds1_filter_4}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/sweeps_ds1_filter_4.pdf}
\caption[Final hyperparameter space mapped to the best validation loss for dataset 1]{\textbf{Final hyperparameter space mapped to the best validation loss for \gls{ds1}.} In four columns, the dropout probability, the hidden size, the number of layers and the weight decay, filter boxes are applied reducing the shown sweeps from a number of 24 to 1.}
\label{fig:sweeps_ds1_filter_4}
\end{figure}

With the second reduction of \autoref{fig:sweeps_ds1_filter_4}, only sweeps with a hidden size of 512, a number of layers of 7 and with a weight decay of 0 are finally considered, yielding a final set of hyperparameters. Finding the best sweep could have been done by just selecting the sweep with the lowest best validation \gls{rmse}, but would not reveal the bad effect of a dropout of 0.5 for this model. Furthermore, the reduction filters are not selected such that the sweep with the lowest best validation loss is left, but with accordance with the other dataset, to find the most common set of parameters that yield the best results for both utilized datasets. \autoref{tab:hyperparameter_final} lists the optimal shared hyperparameters for the two datasets.

\begin{table}[!ht]
\centering
\caption[Optimal shared hyperparameters found via hyperparameter search matching both datasets]{Optimal shared hyperparameters found via hyperparameter search matching both datasets}
\begin{tabular}{ccccc}
\hline
\hline
\addlinespace
Dropout probability & Hidden size & Number of layers & Weight decay\\
\addlinespace
\toprule
\addlinespace
0 & 512 & 7 & 0 \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:hyperparameter_final}
\end{table}\vspace{10pt}

The complete final hyperparameter set is presented in \autoref{tab:hyperparameter_final_full}. It is the optimal hyperparameter set found for the defined grid and selected random seed, however, extending the grid and using different random seeds may lead to even better results. Random seeding is used for reproducibility, but may also influence the success and results of a particular training session as the initialization of the weights and the bias depends on it. Therefore, scientists run their experiments often with different seeds \cite{picard2021torch}.\\

\begin{table}[!ht]
\centering
\caption[Final hyperparameter set for FlexKalmanNet]{Final hyperparameter set for FlexKalmanNet}
\begin{tabular}{l|c}
\hline
\hline
\addlinespace
Hyperparameter & Optimal value \\
\addlinespace
\toprule
\addlinespace
Random seed & 0 \\
Input size & 7 \\
Output size & 20 \\
Batch size & 512 \\
Hidden size & 512 \\
Number of layers & 7 \\
Learning rate & $1e^{-5}$ \\
Dropout probability & 0 \\
Weight decay penalty term & 0 \\
Loss function & \gls{mse} \\
Loss scheduler & \gls{relrop} \\
Loss cut & 100 \\
Optimizer & \gls{adam} \\
Activation function & Leaky\gls{relu} \\
Number of epochs & 100 \\
Early stopping after epochs & 20 \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:hyperparameter_final_full}
\end{table}\vspace{10pt}

In \autoref{fig:training_losses_ds2}, the convergence of the training of \gls{ds2} using the final hyperparameter set is presented. Corresponding plots for \gls{ds1} can be found in the \hyperref[appendix_training]{Appendix A.2}. From \autoref{fig:training_losses_ds2}, it can be derived, that the training is stable and converging fast and hence, that the learning of the parameters is feasible for the applied \gls{dfcnn}. After about six epochs, the model already reaches the convergence phase. In this phase, the loss is still slightly decreasing until epoch 27, where a negative peak in the loss can be observed. 20 epochs later, the training is stopped by the early stopping mechanism, since for 20 epochs, no lower loss than the one from epoch 27 is reached.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/training_losses_ds2.pdf}
\caption[Convergence behavior of the root mean squared error losses during training with dataset 2]{\textbf{Convergence behavior of the \gls{rmse} losses during training with \gls{ds2}.} Two \gls{rmse} losses of each epoch during the training of the \gls{dfcnn} model using \gls{ds2} are presented: The loss from the training phase, blue, and the loss of the validation phase, orange.}
\label{fig:training_losses_ds2}
\end{figure}

To further analyze the stability and convergence of the training and learning, the evolution of the learned noise covariance parameters can be observed in \autoref{fig:training_sigmas_ds2}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/training_sigmas_ds2.pdf}
\caption[Convergence behavior of the learned parameters during training with dataset 2]{\textbf{Convergence behavior of the learned parameters during training with \gls{ds2}.} The 20 noise covariance terms that the \gls{dfcnn} is learning from the \gls{ds2} are tracked over each epoch and depicted in this graph.}
\label{fig:training_sigmas_ds2}
\end{figure}

Similarly to the convergence behavior of the \gls{rmse}, the learned noise covariance parameters start converging at the latest of about six epochs. Thereupon, only slight changes of the parameters are observable. At the best epoch of the training, epoch 27, no remarkable changes in values can be seen. This implies, that the slightly changing parameters form fine-adjusted combinations yielding better and worse results, where at epoch 27 the smallest loss is produced.

In \autoref{tab:training_results}, the final results of the trainings are presented. These results include for each dataset the best validation epoch, the best validation \gls{rmse}, the test \gls{rmse} and the computation time in seconds per epoch, which are measured during trainings deployed on the virtual server (see \autoref{sec:trainaing_scenarios}).\\

\begin{table}[!ht]
\centering
\caption[Final results of the trainings with the best found hyperparameters for each dataset]{Final results of the trainings with the best found hyperparameters for each dataset}
\begin{tabular}{cccccc}
\hline
\hline
\addlinespace
Dataset & Hidden & Best val. &       Best val. &            Test & Computation time \\
        &   size &     epoch & \gls{rmse} loss & \gls{rmse} loss &     in [s/epoch] \\
\addlinespace
\toprule
\addlinespace
\gls{ds1} &  512 & 49 & 0.0059 & 0.0067 & 39.4286 \\
\gls{ds2} &  512 & 27 & 0.0176 & 0.0189 & 41.2500 \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:training_results}
\end{table}\vspace{10pt}

The first thing to notice in \autoref{tab:training_results} is that the losses for both datasets are fairly small, implying high accuracies - further test results of the \gls{ekf}'s accuracies are presented in the subsequent section. In addition, the losses prove that the trained parameters also perform well on unseen data, otherwise the validation and test loss would not be as close as they are in the results.
Furthermore, the losses exhibit that the losses for \gls{ds1} are significantly smaller than those for \gls{ds2}. This difference in losses can be explained by the different magnitues of angular velocities in the data. The moderate angular velocities of \gls{ds1} inherit less changes in the data compared to the data with higher angular velocities, \gls{ds2}. Thus, \gls{ds2} contains more and faster changes in magnitudes which are more difficult to compensate, leading to higher losses. Plots presenting the data and the \gls{ekf}'s sensitivity are given and also analyzed in the subsequent section.

The computation times do not allow for further conclusions. Using \glspl{gpu} for the training to enable parallel computing may lead to faster convergence times, whereby it must be considered, that the bottleneck at some point might be the \gls{ekf} state estimation, which is a process that cannot be distributed in small computational fractions and thus may take even longer when deployed on a \gls{gpu} core instead of a computational faster \gls{cpu} core.

The best validation epochs only allow for the conclusion that the convergence behavior overall is good and fairly fast regarding the complexity of the parameter space being learned.

\autoref{tab:training_results} may additionally serve as a baseline when tuning FlexKalmanNet differently, when applying it to different \glspl{kf} such as the \gls{ukf} or testing other networks like EKFNet or KalmanNet with the same data for comparison.



\section{Evaluation of the Learned Parameters}
To evaluate the \gls{ekf}'s functionality using the learned parameters, the learned parameters for \gls{ds1} and \gls{ds2} are applied in an \gls{ekf} and analyzed. Therefore, offline \gls{ekf} runs using the recorded rosbag data from \gls{ds1} and \gls{ds2} with additive Gaussian noise with a standard deviation of $\sigma = 0.1$ for all measurement features are conducted. The goal is to analyze the learned parameters under the aspects of accuracy, stability, robustness, sensitivity and settling time. Different plots are presented that exhibit different parts for this analysis.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_offline_ds1_ds1.pdf}
\caption[Offline results of the extended Kalman filter using the trained parameters for dataset 1 applied on dataset 1]{\textbf{Offline results of the \gls{ekf} using the trained parameters for \gls{ds1} applied on \gls{ds1}.} Each of the four subplots depicts one of the four spatial motion components from the state vector: The orientation, the position, the angular velocity and the translational velocity. Whereby each of the spatial motion components consists of its own components, such as angular velocities about the three spatial axes, x, y and z. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted. The orientations and positions ground truths contain the additive Gaussian noise that the \gls{ekf} shall filter and are therefore referenced as \textit{measured}.}
\label{fig:ekf_states_offline_ds1_ds1}
\end{figure}

In \autoref{fig:ekf_states_offline_ds1_ds1}, as the first tested combination, an \gls{ekf} with the learned parameters for \gls{ds1} is applied to the corresponding dataset with moderate angular velocities, \gls{ds1}. Results for this run are presented. This first testing demonstrates various functionality aspects. First of all, the \gls{ekf} converges and remains stable over time. Next, all the variables seem to be filtered very well, only small uncertainties around the ground truth of the angular velocities are noticeable. The quaternions exhibit a lot of motion which the \gls{ekf} is sensitive to and has no problem tracking. The \gls{ekf} is also able to follow the angular velocities that change slightly over time. The position and translational velocities, in turn, do not contain any major changes and are thus very stably estimated from the \gls{ekf}. Hence, the \gls{ekf} using the learned parameters for \gls{ds1} seems very promising. Later in this section, the \gls{rmse} and the uncertainty of each component from the state vector are presented. Applying the learned parameters for \gls{ds1} to \gls{ds2}, which contains fast velocities, yields \autoref{fig:ekf_states_offline_ds1_ds2}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_offline_ds1_ds2.pdf}
\caption[Offline results of the extended Kalman filter using the trained parameters for dataset 1 applied on dataset 2]{\textbf{Offline results of the \gls{ekf} using the trained parameters for \gls{ds1} applied on \gls{ds2}.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_offline_ds1_ds2}
\end{figure}

As in \autoref{fig:ekf_states_offline_ds1_ds1}, in \autoref{fig:ekf_states_offline_ds1_ds2} the translational motion is still perfectly stable, even though the ground truth of the translational velocity is more unstable in \gls{ds2} compared to \gls{ds1}. This may be attributed to the controller of the \gls{ars} that has to compensate higher forces when simulating high velocities, leading to higher uncertainties in other motion components. Looking at the subplots of the rotational components, also unstable behavior is observable in the measured data. Still, the \gls{ekf}'s estimate are very smooth and sleek but slightly lagging behind. It seems like the parameters for \gls{ds1} are not perfectly sensitive for the higher dynamics present in \gls{ds2}. Still, the \gls{ekf} using the learned parameters for \gls{ds1} yields fairly good results, also for \gls{ds2}, even though it is trained on \gls{ds1}. The training using \gls{ds2} includes higher angular velocities in the data. \autoref{fig:ekf_states_offline_ds2_ds2} shows the results of applying the \gls{ekf} again to \gls{ds2}, but with the trained parameters for \gls{ds2}.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_offline_ds2_ds2.pdf}
\caption[Offline results of the extended Kalman filter using the trained parameters for dataset 2 applied on dataset 2]{\textbf{Offline results of the \gls{ekf} using the trained parameters for \gls{ds2} applied on \gls{ds1}.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_offline_ds2_ds2}
\end{figure}

In the results of \autoref{fig:ekf_states_offline_ds2_ds2}, the lack of sensitivity for higher changes of rotational features seems to be non-existent anymore. The training with the faster angular velocities of \gls{ds2} leads to parameters that are more sensitive to changes like those present in \gls{ds2}. This implies that if the sensitivity of learned parameters is not high enough, and the simulation of data is possible, data with higher velocities can be used to encourage sensitivity within the learned parameters. For the sensitivity it is crucial that the batch size is large enough to give enough data context, such that dynamics in the data can be captured within each batch. Thus, an alternative to the simulations with high velocities to encourage sensitivity learning would be to increase the batch size providing more data context and thus more potential dynamics to catch and learn to be sensitive for. Higher batch sizes, then again, require more data and computational effort during training.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_offline_ds2_ds1.pdf}
\caption[Offline results of the extended Kalman filter using the trained parameters for dataset 2 applied on dataset 1]{\textbf{Offline results of the \gls{ekf} using the trained parameters for \gls{ds2} applied on \gls{ds1}.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_offline_ds2_ds1}
\end{figure}

In \autoref{fig:ekf_states_offline_ds2_ds1}, the last of the four combinations, the \gls{ekf} using the learned parameters for \gls{ds2} applied to the data with the slower angular velocities, the \gls{ds1}, is presented. As in all of the presented experiments of this section so far, \autoref{fig:ekf_states_offline_ds2_ds1} also exhibits stable behavior, especially for the translational motion. From \autoref{fig:ekf_states_offline_ds2_ds2}, it is concluded, that the learned parameters for \gls{ds2} are more sensitive to changes in the data than the learned parameters for \gls{ds1}. This higher sensitivity seems advantageous, but also has a potential downside as shown in \autoref{fig:ekf_states_offline_ds2_ds1}: The estimates for the angular velocities seem slightly noisy. This can be attributed to a too high sensitivity against noise. In table \autoref{tab:parameters}, the learned parameters for \gls{ds1} and for \gls{ds2} are compared, revealing that for \gls{ds1} indeed higher values for the process noise covariances are learned, which makes the \gls{ekf} more sensitive. Hence, the results from \autoref{tab:parameters} and the offline runs confirm each other. For the parameters it is crucial to strike a balance. Excessively high values for the process noise covariances might cause the filter to overreact to noise, leading to overfitting, while too low values might cause the filter to underfit and not adapt adequately to the system's dynamics \cite{saha2013robustness}.\\

\begin{table}[!ht]
\centering
\caption[Learned standard deviation parameters for dataset 1 and dataset 2]{Learned standard deviation parameters for \gls{ds1} and \gls{ds2}}
\begin{tabular}{c|cc}
\hline
\hline
\addlinespace
  Trained & Learned value & Learned value \\
parameter & for \gls{ds1} & for \gls{ds2} \\
\addlinespace
\toprule
\addlinespace
$\sigma_{R_{q_w}}$ & 0.042746 & 0.045785 \\
$\sigma_{R_{q_x}}$ & 0.036301 & 0.038067 \\
$\sigma_{R_{q_y}}$ & 0.048697 & 0.048149 \\
$\sigma_{R_{q_z}}$ & 0.029550 & 0.035209 \\[4pt]
$\sigma_{R_{s_x}}$ & 0.078810 & 0.073300 \\
$\sigma_{R_{s_y}}$ & 0.058190 & 0.054914 \\
$\sigma_{R_{s_z}}$ & 0.082663 & 0.081457 \\[4pt]
$\sigma_{Q_{q_w}}$ & 0.000161 & 0.000145 \\
$\sigma_{Q_{q_x}}$ & 0.000090 & 0.000667 \\
$\sigma_{Q_{q_y}}$ & 0.000071 & 0.002006 \\
$\sigma_{Q_{q_z}}$ & 0.000026 & 0.000026 \\[4pt]
$\sigma_{Q_{s_x}}$ & 0.000150 & 0.006237 \\
$\sigma_{Q_{s_y}}$ & 0.000010 & 0.004650 \\
$\sigma_{Q_{s_z}}$ & 0.000132 & 0.006365 \\[4pt]
$\sigma_{Q_{\omega_x}}$ & 0.000079 & 0.000575 \\
$\sigma_{Q_{\omega_y}}$ & 0.000145 & 0.000515 \\
$\sigma_{Q_{\omega_z}}$ & 0.000037 & 0.000876 \\[4pt]
$\sigma_{Q_{v_x}}$ & 0.000023 & 0.000087 \\
$\sigma_{Q_{v_y}}$ & 0.000028 & 0.000022 \\
$\sigma_{Q_{v_z}}$ & 0.000025 & 0.000040 \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:parameters}
\end{table}\vspace{10pt}

Another finding of the table with the learned parameters (\autoref{tab:parameters}) is that the parameters for the measurement noise covariances are very similar for both datasets. This means, that the underlying, identical noise can be learned from both datasets. Due to the difference of the present context in each batch, the models adjust the parameters for the process noise covariances to best-fit the present dynamics found in each batch during learning, yielding different sensitivities of the trained models.

Since \gls{ds1} is the more realistic dataset and hence of higher relevance, further tests for the trained parameters from both \gls{ds1} and \gls{ds2} are run on \gls{ds1}. In \autoref{tab:rmse} the \gls{rmse} of both datasets for every state variable computed when run on \gls{ds1} are listed.\\

\begin{table}[!ht]
\centering
\caption[Root mean square errors of each variable of the state vector for extended Kalman filter runs on dataset 1 using learned parameters trained with dataset 1 and dataset 2]{Root mean square errors of each variable of the state vector for \gls{ekf} runs on \gls{ds1} using learned parameters trained with \gls{ds1} and \gls{ds2}}
\begin{tabular}{ccc}
\hline
\hline
\addlinespace
   State & \gls{rmse} & \gls{rmse} \\
variable &  \gls{ds1} &  \gls{ds2} \\
\addlinespace
\toprule
\addlinespace
     $q_w$ & 0.044 & 0.045 \\
     $q_x$ & 0.046 & 0.048 \\
     $q_y$ & 0.039 & 0.039 \\
     $q_z$ & 0.047 & 0.049 \\
     $s_x$ & 0.102 & 0.107 \\
     $s_y$ & 0.103 & 0.107 \\
     $s_z$ & 0.101 & 0.105 \\
$\omega_x$ & 0.001 & 0.004 \\
$\omega_y$ & 0.001 & 0.003 \\
$\omega_z$ & 0.001 & 0.003 \\
     $v_x$ & 0.002 & 0.002 \\
     $v_y$ & 0.001 & 0.002 \\
     $v_z$ & 0.001 & 0.001 \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:rmse}
\end{table}\vspace{10pt}

As observed in the tests so far, the \gls{ekf} runs using the learned parameters of \gls{ds1} are less sensitive to noise and not only well-trained, but also the better fit for \gls{ds1}. \autoref{tab:rmse} concludes these observations by exhibiting that all of the state features are more accurate in the \gls{ds1} run than in the \gls{ds2} run. Still, the trained parameters for \gls{ds2} have very low errors, too. The \gls{rmse} of $w_x$ e.g. is 0.004\,rad/s, which is equivalent to $0.23\hspace{0.1pt}^{\circ}$/s. The overview of the featurewise errors also shows that the features introduced as noisy measurements are exhibiting significant larger \gls{rmse} compared to the derived twist features. This differences may be attributed to the fact that the derived variables (angular and translational velocities) rely more on the dynamics of the system rather than direct on the noisy measurements, as the orientations and positions do.

As another metric for accuracy and stability of the filter, the standard deviations of each feature of the error state of the \gls{ekf} are studied. Therefore, the \gls{ekf} is run on only 500 samples to increase the resolution of the settling phase of the \gls{ekf}. Due to high similarities of the results from the both dataset runs and the highest relevance of \gls{ds1}, only results using the learned parameters for \gls{ds1} and on \gls{ds1} are presented and discussed. The corresponding results for the parameters learned with \gls{ds2} run on \gls{ds1} can be found in the \hyperref[appendix_uncertainties]{Appendix A.3}. The evolution of the uncertainties of the orientations during the \gls{ekf} filtering are shown in \autoref{fig:ekf_uncertainties_orientations_ds1}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_uncertainties_orientations_ds1.pdf}
\caption[Uncertainties of the extended Kalman filter orientation estimates for dataset 1 on dataset 1]{\textbf{Uncertainties of the \gls{ekf} orientation estimates for \gls{ds1} on \gls{ds1}.} Each of the four subplots depicts one of the components of the orientations from the state. In every subplot, the \gls{ekf} estimate, the corresponding ground truth and the uncertainty space are plotted. For the uncertainty space, the double standard deviation of the corresponding error state feature is utilized.}
\label{fig:ekf_uncertainties_orientations_ds1}
\end{figure}

The uncertainty is computed as double standard deviation which represents the space in which the estimate will be in with a probability of 95.4\,\%. \autoref{fig:ekf_uncertainties_orientations_ds1} exhibits sawtooth-like uncertainties for all four quaternion components. These uncertainties decrease strongly within the first 100 discrete-time steps, where the uncertainty boundaries start converging to the estimate. This indicates that the filter becomes very confident about its estimates. The sawtooth-like shape can be attributed to the lack-of-measurement mechanism, which lets the \gls{ekf} propagate (predict) the current state until the next correction based on a measurement is performed. This correction decreases the uncertainty rapidly, whereupon the propagation with lower uncertainty is performed again until the next correction is performed.

Observing the uncertainties of the angular velocities (see \autoref{fig:ekf_uncertainties_angular_velocities_ds1}), again, a strong decrease within the first 100 to 150 discrete-time steps can be seen. This plot additionally allows to analyse the settling time more easily due to the nearly constant ground truth, where the settling time correlates with the phase of strong decrease in state uncertainty. A notable difference to the orientation uncertainties is the smaller magnitude and a smaller increase of the uncertainty during pure propagation phases. This behavior is reflected in \autoref{tab:rmse}, where larger errors can be observed for the pose features. Thus, these flattened and smaller uncertainties can be attributed to the smaller dependency of the velocity terms from the noisy measurements and the higher reliance to the model's dynamics. Plots of the uncertainties of the positions and translational velocities can also be found in the \hyperref[appendix_uncertainties]{Appendix A.3}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_uncertainties_angular_velocities_ds1.pdf}
\caption[Uncertainties of the extended Kalman filter angular velocity estimates for dataset 1 on dataset 1]{\textbf{Uncertainties of the \gls{ekf} angular velocity estimates for \gls{ds1} on \gls{ds1}.} Each of the three subplots depicts one of the components of the angular velocities from the state. In every subplot, the \gls{ekf} estimate, the corresponding ground truth and the uncertainty space are plotted. For the uncertainty space, the double standard deviation of the corresponding error state feature is utilized.}
\label{fig:ekf_uncertainties_angular_velocities_ds1}
\end{figure}

In order to test robustness with respect to noise, the learned parameters from \gls{ds1} and \gls{ds2} are tested on \gls{ds1} with an increased noise of a magnitude five times larger than existent in the data during the training: $\sigma = 0.5$. \autoref{fig:ekf_states_noise_5_ds1} depicts the results of the \gls{ekf} run with the \gls{ds1} parameters applying the increased noise in the data.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_noise_5_ds1.pdf}
\caption[Extended Kalman filter offline results for the trained dataset 1 parameters on dataset 1 with five times larger noise magnitude]{\textbf{\Gls{ekf} offline results for the trained \gls{ds1} parameters on \gls{ds1} with five times larger noise magnitude.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_noise_5_ds1}
\end{figure}

The large noise can be seen in the ground truth of the orientation and position subplots of \autoref{fig:ekf_states_noise_5_ds1}. Even though the magnitude of the noise is five times larger, the translational components are still very stable. The rotational components, in turn, start exhibiting uncertainties for the angular velocity estimates, whereby these are still in a relatively small range and thus still accurate when considering the excessive increase of noise.\\

For the learned parameters of \gls{ds2}, all components of the state vector become noisy, see \autoref{fig:ekf_states_noise_5_ds2}. These components are more sensitive to noise as discovered earlier in this section and thus not capable to handle larger noises while remaining stable estimates.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_noise_5_ds2.pdf}
\caption[Extended Kalman filter offline results for the trained dataset 2 parameters on dataset 1 with five times larger noise magnitude]{\textbf{\Gls{ekf} offline results for the trained \gls{ds2} parameters on \gls{ds1} with five times larger noise magnitude.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_noise_5_ds2}
\end{figure}

When analyzing the robustness in terms of varying noise, also the behavior of the \gls{ekf} for data with less noise than originally learned is to be tested. Therefore, the learned parameters are tested again on \gls{ds1} with no additive noise in the data: $\sigma = 0$. Since the results are visually not distinguishable, again, only the results of the \gls{ekf} run using the parameters from \gls{ds1} are presented, see \autoref{fig:ekf_states_noise_0_ds1}. The results for \gls{ds2} can be found in the \hyperref[appendix_noise_free]{Appendix A.4}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_noise_0_ds1.pdf}
\caption[Extended Kalman filter offline results for the trained dataset 1 parameters on dataset 1 with no additive noise]{\textbf{\Gls{ekf} offline results for the trained \gls{ds1} parameters on \gls{ds1} with no additive noise.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_noise_0_ds1}
\end{figure}

The results for the noise-free tests prove in \autoref{fig:ekf_states_noise_0_ds1} that when the data's noise decreases, the \gls{ekf} remains very stable. Also, the uncertainty caused by the high sensitivity against noise existent in the parameters of the parameters learned from \gls{ds2} is vanishing if there is no noise.\\

As final test, the stability of the \gls{ekf} is put to the test by increasing the lack of measurements to 100 discrete-time step. Thereby, scenarios where the measurement update rates are low or may drop to a low rate are simulated. \autoref{fig:ekf_states_steps_100_ds1} presents the results of this stability test of the trained parameters from \gls{ds1} on \gls{ds1}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_steps_100_ds1.pdf}
\caption[Extended Kalman filter offline results for the trained dataset 1 parameters on dataset 1 with increased lack of data]{\textbf{\Gls{ekf} offline results for the trained \gls{ds1} parameters on \gls{ds1} with increased lack of data.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted. The square-like shapes in the data are caused by an introduced lack of data of a discrete-time step size of 100.}
\label{fig:ekf_states_steps_100_ds1}
\end{figure}

In \autoref{fig:ekf_states_steps_100_ds1}, it can be seen that the settling time seems to be increased, but the filter remains totally stable over time. Hence, the stability of the \gls{ekf} is not endangered by missing data. Also in \autoref{fig:ekf_states_steps_100_ds2}, where the parameters from the \gls{ds2} training are tested on \gls{ds1}, the stability does not decrease.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_steps_100_ds2.pdf}
\caption[Extended Kalman filter offline results for the trained dataset 2 parameters on dataset 1 with increased lack of data]{\textbf{\Gls{ekf} offline results for the trained \gls{ds2} on \gls{ds1} with increased lack of data.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted. The square-like shapes in the data are caused by an introduced lack of data of a discrete-time step size of 100.}
\label{fig:ekf_states_steps_100_ds2}
\end{figure}

The plots of the simulations of an increased lack of data, \autoref{fig:ekf_states_steps_100_ds2}, approve again the stability and robustness of the learned parameters. 



\clearpage
\section{Verification of the Online Functionality}
In order to verify the \gls{ekf}'s online functionality using the trained parameters for both datasets while testing the implemented \gls{ros} package, the \gls{ekf} is additionally run online in the implemented \gls{ros} package using the \gls{ars} and the realistic and moderate angular velocities applied in \gls{ds1} (see \autoref{sec:data_generation}). For analysis, the angular velocities are presented as representative features. Plots for the remaining state features can be found in the \hyperref[appendix_online_tests]{Appendix A.5}.

\autoref{fig:ekf_states_online_ds1_stability_angular_velocities} depicts the stability of the angular velocity features for the trained parameters from \gls{ds1}. It can be seen, that the estimates are stable over time while slightly lagging behind the true values, which is visible in this plot due to the high resolution of the y-axis, as the settling time is excluded in this plot.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_online_ds1_stability_angular_velocities.png}
\caption[Extended Kalman filter online stability results for the angular velocity state features using the trained parameters from dataset 1 and data equal to dataset 1 with no additive noise]{\textbf{\Gls{ekf} online stability results for the angular velocity state features using the trained parameters from \gls{ds1} and data equal to \gls{ds1} with no additive noise.} Each of the 3 subplots depicts one of the three angular velocity components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_online_ds1_stability_angular_velocities}
\end{figure}

Comparing these results to \autoref{fig:ekf_states_online_ds2_stability_angular_velocities}, which shows the corresponding results for the trained parameters with \gls{ds2}, again the higher sensitivity of these parameters can be seen. Due to the higher sensitivity, the \gls{ekf} manages also in this small scope to estimate the angular velocities with barely no lag, with the price of having less stable estimates for the angular velocities and also for the positions.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_online_ds2_stability_angular_velocities.png}
\caption[Extended Kalman filter online stability results for the angular velocity state features using the trained parameters from dataset 2 and data equal to dataset 1 with no additive noise]{\textbf{\Gls{ekf} online stability results for the angular velocity state features using the trained parameters from \gls{ds2} and data equal to \gls{ds1} with no additive noise.} Each of the 3 subplots depicts one of the three angular velocity components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_online_ds2_stability_angular_velocities}
\end{figure}

Due to similarities of the settling time analysis, only the results of the trained parameters for \gls{ds1} are presented, see \autoref{fig:ekf_states_online_ds1_settling_angular_velocities}. The results for the trained parameters of \gls{ds2} can be found in the \hyperref[appendix_online_tests]{Appendix A.5}. \autoref{fig:ekf_states_online_ds1_settling_angular_velocities} demonstrates, that the settling time matches with the observations of the offline tests: Within 10 to 15\,s, the state variables converge, which is sufficiently fast for rendezvous operations \cite{fehse2003automated}. The offline and online results yield the same conclusions which verifies the online applicability of the learned \gls{ekf} parameters and the functionality of the \gls{ros} package whereby the data source for the online and offline runs is the same, after all.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_online_ds1_settling_angular_velocities.png}
\caption[Extended Kalman filter online settling time results for the angular velocity state features using the trained parameters from dataset 1 and data equal to dataset 1 with no additive noise]{\textbf{\Gls{ekf} online settling time results for the angular velocity state features using the trained parameters from \gls{ds1} and data equal to \gls{ds1} with no additive noise.} Each of the 3 subplots depicts one of the three angular velocity components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_online_ds1_settling_angular_velocities}
\end{figure}



\clearpage
\section{FlexKalmanNet Versus Manual Tuning}
FlexKalmanNet enables to use the trained noise covariance parameters for an \gls{ekf} from the training instead of having to find and tune the parameters manually. To evaluate the performance of the trained parameters, as a baseline, a manually tuned \gls{ekf} is tested (chosen parameters are presented in \autoref{sec:test_eval_metrics}). The results of an \gls{ekf} run using the manually tuned parameters on the closest to real-life data scenario, \gls{ds1}, are depicted in \autoref{fig:ekf_states_manually_tuned_ds1}.\\

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/ekf_states_manually_tuned_ds1.pdf}
\caption[Extended Kalman filter offline results for manually tuned parameters run on dataset 1]{\textbf{\Gls{ekf} offline results for manually tuned parameters run on \gls{ds1}.} Each of the four subplots depicts one of the four spatial motion components from the state vector. In every subplot, the \gls{ekf} estimate and the corresponding ground truth are plotted.}
\label{fig:ekf_states_manually_tuned_ds1}
\end{figure}

In \autoref{fig:ekf_states_manually_tuned_ds1}, it can be seen that the initial guess for the \gls{ekf} using manually tuned parameters produces qualitatively good matching estimates for the translational components. Also the results for the rotational components are comparably good considering the usage of the first trial of the manually tuned parameters. A reduction of the process covariance entries may lead to less sensitivity against the noise and thus to better results. This manual tuning procedure is exactly the operation to be replaced by FlexKalmanNet. Furthermore, the tuning applied already involves the true standard deviation of the measurement noise, which often is not available and therefore the FlexKalmanNet is supposed to find out.

In addition to \autoref{fig:ekf_states_manually_tuned_ds1}, \autoref{tab:manual} presents the \gls{rmse} of the manually tuned offline \gls{ekf} run and of the learned parameter from \gls{ds1} \gls{ekf} run, both applied to \gls{ds1}, to compare the performance.\\

\begin{table}[!ht]
\centering
\caption[Root mean square errors of each variable of the state vector for extended Kalman filter runs using learned parameters from dataset 1 and using the manually tuned parameters, both run on dataset 1]{Root mean square errors of each variable of the state vector for \gls{ekf} runs using learned parameters from \gls{ds1} and using the manually tuned parameters, both run on \gls{ds1}}
\begin{tabular}{ccc}
\hline
\hline
\addlinespace
   State & \gls{rmse} &    \gls{rmse} \\
variable &  \gls{ds1} & manual tuning \\
\addlinespace
\toprule
     $q_w$ & 0.044 & 0.047 \\
     $q_x$ & 0.046 & 0.050 \\
     $q_y$ & 0.039 & 0.041 \\
     $q_z$ & 0.047 & 0.052 \\
     $s_x$ & 0.102 & 0.103 \\
     $s_y$ & 0.103 & 0.103 \\
     $s_z$ & 0.101 & 0.103 \\
$\omega_x$ & 0.001 & 0.008 \\
$\omega_y$ & 0.001 & 0.008 \\
$\omega_z$ & 0.001 & 0.008 \\
     $v_x$ & 0.002 & 0.002 \\
     $v_y$ & 0.001 & 0.001 \\
     $v_z$ & 0.001 & 0.001 \\
\addlinespace
\hline
\hline
\end{tabular}
\label{tab:manual}
\end{table}\vspace{10pt}

\autoref{tab:manual} exhibits that the \gls{rmse} of all features of the estimated state of the \gls{ekf} run using the trained parameters from \gls{ds1} are less or equal to those of the \gls{ekf} run using the manually tuned parameters. Especially the rotational components whose dynamics are based on linearizations and thus more complicated to tune are all more accurate when using the trained parameters. The translational features are quite similar, proving that the initial estimate for the manually tuned parameters of the translational motion is well selected and thus that the dynamics of the translational motion can be assumed to be accurate.


==> text/XX_theoretical_fundamentals.tex <==
\section{Motion Dynamics}
Depending on the system of interest and all assumptions that build its boundaries, motion dynamics can be described using different representations. In the context of this work, the motion descriptions are presenting the motion dynamic equations in the form of one-step-ahead estimators. A one-step-ahead estimator is a predictive framework that provides estimates of future values or states based on current information, with a focus on making predictions for the immediate next time step \cite{crassidis2011optimal}. Its recursive nature allows for continuous updates and adjustments as new data is collected, making it a valuable tool in real-time prediction processes. The domain of interest for this work, and several principal motion representations are presented in this section.

In the equations of this section, many notations can be found. The most of them are clarified when presented for the first time. However, all notations can be found in the list of symbols.


\subsection{Close-Proximity Relative Motion Space Operations}
In the context of space dynamics, close-proximity operations refer to scenarios where two or more space objects are in close proximity to each other, such as docking maneuvers. The motion dynamics in such scenarios are crucially important for the safety and success of the executed maneuver \cite{ankersen2010guidance}.

If there are two objects involved in a rendezvous or docking maneuver, an active one and a passive one, the active object, a spacecraft, is called the \textit{chaser} and the passive object is called the \textit{target} \cite{bonnal2013active}. The first challenge for rendezvous space operations is the orbital synchronization between the chaser and the target. For this operation, accurate orbital mechanics calculus is required to align the spacecraft's orbit accurately to the target's orbit while maintaining a safe distance. Therefore, the relative motion dynamics are required. It is the \textit{relative} motion that is essential because their movements are described in relation to each other rather than with respect to an external reference frame. This makes controlling and maneuvering more straightforward, as the chaser can adjust its trajectory and orientation based on the relative motion and pose of the target. When the chaser is in the desired close range of the target having a relative translational velocity of zero, close-proximity operations can be conducted \cite{luo2014survey}.

Key instruments used for relative navigation include sensors such as cameras, \gls{lidar} \cite{christian2013survey}, radar, and \gls{gps} receivers. These sensors provide data that is processed by the spacecraft's \gls{gnc} system to continually update the relative position and motion information. This real-time information is necessary for making decisions about the spacecraft's trajectory autonomously and ensuring a collision-free and accurate approach during a docking process \cite{reesman2018getting}.


\subsection{Translational Motion Dynamics of Discrete-Time Systems}
Translational motion is the simplest form of motion, involving the movement of an object from one point to another without any change in orientation or rotation. It forms the basis for understanding how objects move in space and serves as the foundation for understanding more complex types of motion. In simple linear systems, such as the equations of translational motion, often referred to as the equations of motion, the discrete translational motion dynamics can be described as follows \cite{serway2018physics}:

\begin{equation}
\boldsymbol{s}_{k} = \boldsymbol{s}_{k-1} + \boldsymbol{v}_{k} \Delta t + \boldsymbol{a}_{k} {\Delta t}^{2}
\label{eq:motion_linear_way}
\end{equation}
\begin{equation}
\boldsymbol{v}_{k} = \boldsymbol{v}_{k-1} + \boldsymbol{a}_{k} \Delta t
\label{eq:motion_linear_velocity}
\end{equation}
\begin{equation}
\boldsymbol{a}_{k} = \boldsymbol{a}_{k-1} \\[1.25em]
\label{eq:motion_linear_acceleration}
\end{equation}

Where $\boldsymbol{s}$, $\boldsymbol{v}$ and $\boldsymbol{a}$ are the positions, velocities and accelerations of current and of the previous discrete-time steps $k$ and $k-1$. $\Delta t$ is the time between two subsequent discrete-time steps. In 3D, the position, velocity and acceleration vectors consists of three components that correspond to the x-, y- and z-axis:

\begin{equation}
\boldsymbol{s} = [s_{x}, s_{y}, s_{z}]^{T}
\label{eq:position_components}
\end{equation}
\begin{equation}
\boldsymbol{v} = [v_{x}, v_{y}, v_{z}]^{T}
\label{eq:velocity_components}
\end{equation}
\begin{equation}
\boldsymbol{a} = [a_{x}, a_{y}, a_{z}]^{T} \\[1.25em]
\label{eq:acceleration_components}
\end{equation}


\subsection{Rotational Motion Dynamics of Discrete-Time Systems}
Rotational motion is the motion of an object around a fixed axis. It is fundamental to understanding how objects spin, rotate, or turn, and it complements the translational motion of the previous section. Rotations can be described via different representations. Therefore, e.g. the \textit{Euler rotations}, \textit{Euler axis and angle}, \textit{rotation matrix}, \textit{quaternions}, or multiple other representations can be used \cite{crassidis2011optimal}. Each representation has its advantages and disadvantages. In space technology, quaternions are mostly used since they bring several advantages over other methods \cite{mukundan2012quaternions}:

\begin{itemize}
    \item No Gimbal Lock: One of the most significant advantages of quaternions is that they do not suffer from gimbal lock, unlike Euler angles. Gimbal lock occurs when certain orientations cause the loss of one degree of freedom in a three-dimensional rotational system, making it challenging to represent all possible rotations and resulting in ambiguities.
    \item Memory Efficiency: Quaternions are more memory-efficient compared to rotation matrices, which require nine values (3x3 matrix) to represent a 3D rotation. Quaternions only require four values (a scalar and a 3D vector), making them a more compact representation.
    \item Numerical Stability: Quaternion operations, such as multiplication and normalization, tend to be more numerically stable than operations on rotation matrices.
    \item Efficient Computation: Quaternion multiplication is computationally efficient and can be faster than performing matrix multiplications, especially in cases where you need to apply multiple rotations sequentially.
    \item Global Rotations: Quaternions are particularly useful for representing global rotations, where the order of rotation matters less than it does with Euler angles.
    \item Easily Convertible: Quaternions can be converted to and from rotation matrices and Euler angles, allowing you to work with different representations as needed while still benefiting from the advantages of quaternions when necessary.
\end{itemize}

The main downside of using quaternions is, that they are less intuitive to work with compared to Euler angles. Nevertheless, their mathematical properties make them a powerful tool for representing and manipulating 3D rotations.

In general, a quaternion $\boldsymbol{q}$ is a four-component tuple consisting of $q_{w}$, $q_{x}$, $q_{y}$ and $q_{z}$, where $q_{w}$ is its scalar (real) part and $q_{x}$, $q_{y}$, $q_{z}$ is its vector (imaginary) part. $q_{x}$, $q_{y}$ and $q_{z}$ are the components that build the quaternion's axis of rotation. The scalar part provides information about how much rotation occurs around the specified axis of rotation. Together, these components encode both the axis of rotation and the magnitude of the rotation.

There are two main conventions how a quaternion is being built \cite{sola2017quaternion}.

\begin{itemize}
    \item In the Hamiltonian quaternion convention, quaternions are represented as $\boldsymbol{q} = [q_{x}, q_{y}, q_{z}, q_{w}]$, having the scalar part as the last component.
    \item In the \gls{jpl} quaternion convention, quaternions are represented as $\boldsymbol{q} = [q_{w}, q_{x}, q_{y}, q_{z}]$, having the scalar part as the first component.
\end{itemize}

The \gls{jpl} convention is mostly used in aerospace engineering and robotics and so it is in this work. Hence, in this work, a quaternion has the form:

\begin{equation}
\boldsymbol{q} = [q_{w}, q_{x}, q_{y}, q_{z}]^{T} \\[1.25em]
\label{eq:quaternion_general}
\end{equation}

If the scalar part $q_{w}$ is equal to 0, the quaternion becomes a so-called pure quaternion \cite{dai2015euler}:

\begin{equation}
\boldsymbol{q} = [0, q_{x}, q_{y}, q_{z}]^{T} \\[1.25em]
\label{eq:quaternion_pure}
\end{equation}

Quaternions do not obey the properties of linearity or superposition that are characteristic of vectors in a linear vector space. Quaternions have their own algebraic rules, including quaternion normalization, multiplication, and conjugation. These rules make quaternions suitable for representing and performing operations involving rotations in three-dimensional space, but they are fundamentally different from the linearity and superposition properties found in linear vector spaces. 

Normalizing a quaternion yields a so-called unit quaternion. Unit quaternions are quaternions with a magnitude (L2 norm) of 1 \cite{voight2021quaternion}:

\begin{equation}
||\boldsymbol{q}|| = \sqrt{q_{w}^{2} + q_{x}^{2} + q_{y}^{2} + q_{z}^{2}} \\[1.25em]
\label{eq:quaternion_norm}
\end{equation}

It is advantageous using unit quatenrions due to their numerical stability. Their normalization ensures that they remain stable under numerical operations. In contrast, non-unit quaternions can suffer from drift or instability over time due to accumulation of numerical errors.

When multiple rotations are applied sequentially, the order of the rotations matters. Generally, the composition of rotations is not commutative, meaning that the result depends on the order in which the rotations are applied. Using quaternions, in turn, enables to define a rotation quaternion that can be added iteratively to produce quaternions representing one or multiple continuous and constant rotations. To combine or sum up the orientations of two quaternions, the quaternion multiplication, also called \textit{Hamilton product}, is required, which is denoted using the tensor product operator $\otimes$ \cite{razon1991tensor}, \cite{voight2021quaternion}:

\begin{equation}
\boldsymbol{q}_{1} \otimes \boldsymbol{q}_{2} =
\begin{bmatrix}
q_{1_w} q_{2_w} - q_{1_x} q_{2_x} - q_{1_y} q_{2_y} - q_{1_z} q_{2_z} \\
q_{1_w} q_{2_x} + q_{1_x} q_{2_w} + q_{1_y} q_{2_z} - q_{1_z} q_{2_y} \\
q_{1_w} q_{2_y} - q_{1_x} q_{2_z} + q_{1_y} q_{2_w} + q_{1_z} q_{2_x} \\
q_{1_w} q_{2_z} + q_{1_x} q_{2_y} - q_{1_y} q_{2_x} + q_{1_z} q_{2_w} \\
\end{bmatrix} \\[1.25em]
\label{eq:quaternion_mutliplication}
\end{equation}

Quaternion multiplication allows to combine the rotations represented by the two quaternions into a single quaternion that represents the combined rotation. For subtraction of rotations in quaternion space, quaternion multiplication with the inverse of the second quaternion can be applied.

Using only unit quaternions, the inverse of a quaternions equals the conjugate of a quaternions, which represents the opposite rotation of the original quaternion and is defined as \cite{voight2021quaternion}:

\begin{equation}
\bar{\boldsymbol{q}} = [q_{w}, -q_{x}, -q_{y}, -q_{z}]^{T} \\[1.25em]
\label{eq:quaternion_conjugate}
\end{equation}

The angular velocities $\boldsymbol\omega$ are represented via a vector consisting of three components: $\omega_x$, $\omega_y$ and $\omega_z$, representing the angular velocities around the respective axes:

\begin{equation}
\boldsymbol\omega = {[\omega_x, \omega_y, \omega_z]}^T \\[1.25em]
\label{eq:angular_velocities}
\end{equation}

Accordingly, the angular accelerations $\boldsymbol\alpha$ with $\alpha_x$, $\alpha_y$ and $\alpha_z$ for each axis is defined as a vector:

\begin{equation}
\boldsymbol\alpha = {[\alpha_x, \alpha_y, \alpha_z]}^T \\[1.25em]
\label{eq:angular_accelerations}
\end{equation}

Since for Kalman filters, which are explained in later in this chapter, the model of the dynamic system must be linear \cite{barfoot2011pose}, the Taylor expansion \cite{foy1976position} is applied to linearize the motion dynamics for quaternions:

\begin{equation}
\boldsymbol{q}_{k} = \boldsymbol{q}_{k-1} + \dot{\boldsymbol{q}}_{k-1}\Delta t + \frac{1}{2!}\ddot{\boldsymbol{q}}_{k-1}\Delta t^{2} + \frac{1}{3!}\dddot{\boldsymbol{q}}_{k-1}\Delta t^3 + \cdots \\[1.25em]
\label{eq:quaternion_estimator_taylor_full}
\end{equation}

$\dot{\boldsymbol{q}}$, $\ddot{\boldsymbol{q}}$ and $\dddot{\boldsymbol{q}}$ are the first, second and third derivative of the quaternion. The more orders are taken into account, the better the approximation of the linearization becomes. At the same time, when using higher orders, the computational demand increases rapidly, while the gain in accuracy diminishes with each subsequent increase in order. Hence, to avoid non-linear terms and reduce computational demand while assuming no angular acceleration, only the first-order Taylor expansion is regarded for this work, resulting in:

\begin{equation}
\boldsymbol{q}_{k} = \boldsymbol{q}_{k-1} + \dot{\boldsymbol{q}}_{k-1} \Delta t \\[1.25em]
\label{eq:quaternion_estimator_taylor_short}
\end{equation}

According to Farsoni et al. \cite{farsoni2017compensation}, the first quaternion derivative $\dot{\boldsymbol{q}}$ is defined as:

\begin{equation}
\begin{split}
    \dot{\boldsymbol{q}}(t) &= \underset{\Delta t\to 0}{{lim}} \frac{\boldsymbol{q}(t+\Delta t) - \boldsymbol{q}(t)}{\Delta t} \\
    &= \frac{1}{2} \boldsymbol{q} \otimes [0, \boldsymbol\omega_{bf}]^{T} = \frac{1}{2} [0, \boldsymbol\omega_{wf}]^{T} \otimes \boldsymbol{q} \\
    &= \frac{1}{2} \boldsymbol\Omega \boldsymbol{q} = \frac{1}{2} \boldsymbol\Theta \boldsymbol\omega \\[1.25em]
\end{split}
\label{eq:quaternion_estimator_derivative}
\end{equation}

Where $\boldsymbol\omega_{bf}$ and $\boldsymbol\omega_{wf}$ are the angular velocities vectors in the body frame and in the world frame, $\boldsymbol\Omega$ and $\boldsymbol\Theta$ are matrices that replace the quaternion multiplication with a matrix multiplication, thereby mapping to $\boldsymbol{q}$ and to $\boldsymbol\omega$, respectively. 

For the body frame, $\boldsymbol\Omega_{bf}$ is introduced as:

\begin{equation}
\boldsymbol\Omega_{bf} =
\begin{bmatrix}
       0 & -\omega_x & -\omega_y & -\omega_z \\
\omega_x &         0 &  \omega_z & -\omega_y \\
\omega_y & -\omega_z &         0 &  \omega_x \\
\omega_z &  \omega_y & -\omega_x &         0
\end{bmatrix} \\[1.25em]
\label{eq:quaternion_Omega_bf}
\end{equation}

and $\boldsymbol\Theta_{bf}$ as:

\begin{equation}
\boldsymbol\Theta_{bf} = 
\begin{bmatrix}
-q_{x} & -q_{y} & -q_{z} \\
 q_{w} & -q_{z} &  q_{y} \\
 q_{z} &  q_{w} & -q_{x} \\
-q_{y} &  q_{x} &  q_{w}
\end{bmatrix} \\[1.25em]
\label{eq:quaternion_theta_bf}
\end{equation}

For the world frame, $\boldsymbol\Omega_{wf}$ is defined as:

\begin{equation}
\boldsymbol\Omega_{wf} =
\begin{bmatrix}
       0 & -\omega_x & -\omega_y & -\omega_z \\
\omega_x &         0 & -\omega_z &  \omega_y \\
\omega_y &  \omega_z &         0 & -\omega_x \\
\omega_z & -\omega_y &  \omega_x &         0
\end{bmatrix} \\[1.25em]
\label{eq:quaternion_Omega_wf}
\end{equation}

and $\boldsymbol\Theta_{wf}$ as:

\begin{equation}
\boldsymbol\Theta_{wf} = 
\begin{bmatrix}
-q_{x} & -q_{y} & -q_{z} \\
 q_{w} &  q_{z} & -q_{y} \\
-q_{z} &  q_{w} &  q_{x} \\
 q_{y} & -q_{x} &  q_{w}
\end{bmatrix} \\[1.25em]
\label{eq:quaternion_theta_wf}
\end{equation}

Since for this work measurements and estimations in the world frame are considered, \autoref{eq:quaternion_Omega_wf} and \autoref{eq:quaternion_theta_wf} are utilized for the further derivations.

For state representations that represent not only the orientation but also to the first-order derivative of it (the angular velocities), the second addend of the motion equation should involve the first-order derivative as multiplier to facilitate the extraction of the state vector, similar to \autoref{eq:motion_linear_way}. Therefore, the derivative representation using \autoref{eq:quaternion_theta_wf} is inserted into \autoref{eq:quaternion_estimator_taylor_short}, resulting in the discrete-time linearized motion dynamics for quaternions:

\begin{equation}
\boldsymbol{q}_{k} = \boldsymbol{q}_{k-1} + \frac{\Delta t}{2} \boldsymbol\Theta_{{wf}_{k-1}} \boldsymbol{\omega}_{k-1} \\[1.25em]
\label{eq:quaternion_estimator_q}
\end{equation}

Assuming a constant angular velocity, the evolution of the angular velocities can be computed similarly to \autoref{eq:motion_linear_velocity}, leaving out the acceleration term:

\begin{equation}
\boldsymbol\omega_{k} = \boldsymbol\omega_{k-1}
\label{eq:quaternion_estimator_w} \\[1.25em]
\end{equation}


\subsection{Combined Translational and Rotational Motion Description}\label{sec:dual_quaternions}
In order to combine translational and rotational motion, dual quaternions \cite{perez2004dual} can be used. Dual quaternions are an extension of traditional quaternions, where each dual quaternion consists of two parts: a real part (similar to the scalar part of a quaternion) and a dual part (similar to the vector part of a quaternion). Dual quaternions inherit the advantages of quaternions and are called unit dual quaternions when the real part is normalized to a norm equal to 1. A dual quaternion $\breve{\boldsymbol{q}}$ is defined as \cite{perez2004dual}:

\begin{equation}
\breve{\boldsymbol{q}} = \boldsymbol{q}_r + \epsilon \boldsymbol{q}_d \\[1.25em]
\label{eq:dual_quaternion}
\end{equation}

where $\boldsymbol{q}_r$ and $\boldsymbol{q}_d$ are quaternions representing is the real part and the dual part. $\epsilon$ is the dual unit with the property that $\epsilon^{2} = 0$ but $\epsilon \neq 0$.

To represent combined translational motion and from rotational motion using dual quaternions, two dual quaternions can be composed: A dual quaternion representing the pose $\breve{\boldsymbol{q}}_{pose}$ and a dual quaternion representing the twist $\breve{\boldsymbol{q}}_{twist}$. Therefore, the dual quaternion components must be computed. If the translation is represented in the body frame, the following equation must be used \cite{lee2012dual}:

\begin{equation}
\breve{\boldsymbol{q}} = \boldsymbol{r} + \epsilon \frac{1}{2} \boldsymbol{r} \otimes \boldsymbol{t}_{bf} \\[1.25em]
\label{eq:dual_quaternion_components_bf}
\end{equation}

Where $\boldsymbol{r}$ is a unit or pure rotation quaternion and $\boldsymbol{t}_{bf}$ is pure translation quaternion in the body frame. Similarly, for a pure translation quaternion in the world frame $\boldsymbol{t}_{wf}$, a dual quaternion can be computed via the following equation \cite{lee2012dual}:

\begin{equation}
\breve{\boldsymbol{q}} = \boldsymbol{r} + \epsilon \frac{1}{2} \boldsymbol{t}_{wf} \otimes \boldsymbol{r} \\[1.25em]
\label{eq:dual_quaternion_components_wf}
\end{equation}

Since for this work measurements and estimations in the world frame are considered, \autoref{eq:dual_quaternion_components_wf} is utilized for the computation of dual quaternions.

Given a state that includes the position, the orientation as quaternion, the translational velocity and the angular velocity of a target, the dual quaternion for the pose $\breve{\boldsymbol{q}}_{pose}$ can be composed by using the normalized orientation for the unit quaternion $\boldsymbol{r}$ and the position for the pure quaternion $\boldsymbol{t}_{wf}$ in \autoref{eq:dual_quaternion_components_wf}:

\begin{equation}
\breve{\boldsymbol{q}}_{pose} = [q_{w}, q_{x}, q_{y}, q_{z}]^{T} + \epsilon \frac{1}{2} [0, s_x, s_y, s_z]^{T} \otimes [q_{w}, q_{x}, q_{y}, q_{z}]^{T} \\[1.25em]
\label{eq:dual_quaternion_pose_wf}
\end{equation}

Similarly, the dual quaternion for the twist can accordingly be built using the angular velocity as pure quaternion for $\boldsymbol{r}$ and the translational velocity as pure quaternion for $\boldsymbol{t}_{wf}$ in \autoref{eq:dual_quaternion_components_wf}:

\begin{equation}
\breve{\boldsymbol{q}}_{twist} = [0, \omega_x, \omega_y, \omega_z]^{T} + \epsilon \frac{1}{2} [0, v_x, v_y, v_z]^{T} \otimes [0, \omega_x, \omega_y, \omega_z]^{T} \\[1.25em]
\label{eq:dual_quaternion_twist_wf}
\end{equation}

Further insights into the properties and mathematical operations of dual quaternions are given in the literature \cite{lee2012dual}.


\section{Advanced Filtering}
\Gls{af} of signals refers to the use of sophisticated filtering techniques and algorithms to process and analyze signals, typically in the context of signal processing, communication systems, control systems, and various scientific and engineering applications \cite{thrun2002probabilistic}. \Gls{af} methods go beyond basic filtering approaches, such as simple low-pass, high-pass, or band-pass filters, to address more complex signal processing challenges \cite{deb2015advanced}.

Many applied \gls{af} techniques, are based on algorithms called \gls{ls}, \gls{pf}, and \gls{kf}. These are methods used for estimating unknown states or parameters in dynamic systems, leveraging mathematical models and observed data to refine their estimates over time or through multiple measurements \cite{crassidis2011optimal}.

This section provides the ideas of common state estimators, whereby the \gls{kf} and some extensions of it are presented in more detail since one of them is applied later in this work for the motion estimation algorithm.


\subsection{Common State Estimators}
Three commonly applied state estimators (\gls{ls}, \gls{pf} and \gls{kf}) \cite{sarkka2023bayesian}, \cite{mehmood2012review} are briefly presented in this section to provide an overview about state estimators.


\paragraph{Least Squares}
\Gls{ls} is a method used to estimate unknown parameters or signals from noisy measurements by minimizing the sum of squared errors between the observed data and a model. This technique can be applied for various tasks like regression analysis, system identification, or curve fitting, to obtain accurate parameter estimates in the presence of noise. \Gls{ls} involves solving a batch problem, where all data points are used simultaneously to estimate parameters \cite{crassidis2011optimal}. Therefore, it can only be used for offline scenarios. For online scenarios, recursive extensions like \gls{rls} \cite{engel2004kernel} or \gls{erls} \cite{chen2004extended} for non-linear systems can be applied.


\paragraph{Particle Filter}
The \gls{pf}, also known as the Monte Carlo filter, is an advanced recursive Bayesian filter used for state estimation in dynamic systems. It represents the probability distribution of the system's state using a set of particles (samples). These particles are propagated through the system model, weighted according to their likelihood of being correct based on observed data, and resampled to update the estimate. \Glspl{pf} are especially valuable in non-linear and non-Gaussian state estimation problems, such as tracking moving objects in robotics and sensor fusion. Due to the likelihood computation of each particle and the resampling, the computational demand must be considered \cite{crassidis2011optimal}.


\paragraph{Kalman Filter}
The \gls{kf} is an optimal recursive estimation technique used for state estimation and noise reduction in linear dynamic systems. It employs a mathematical model of the system and the noise and combines predictions with noisy measurements to estimate the state of the system accurately. The \gls{kf} adjusts its estimates over time by iteratively predicting and correcting the state estimate and error covariance matrix in two steps. In those iterations where no new measurement is available, only the prediction is conducted, propagating the estimate purely based on the current state and the system dynamics \cite{welch1995introduction}, \cite{crassidis2011optimal}.

For the \gls{kf} to work, the dynamic system must be linear and the noise normal distributed. For the noise, two separate sources are considered: The process noise and the measurement noise. The process noise describes inaccuracies of the model due to simplifications, such as the neglection of drag, the measurement noise tells how noisy the measurements are. The \gls{kf}'s recursiveness, the consideration of two separate noise sources and the computational efficiency make the \gls{kf} very suitable for real-time applications on embedded systems for complex dynamic systems, like navigation, control systems or tracking \cite{auger2013industrial}.

In case of having a dynamic system that is linear in nature, the \gls{kf} can be applied to it and can also be referred to as \gls{lkf}. If the dynamic system is non-linear, extensions of the \gls{kf}, such as the \gls{ekf} or \gls{ukf} can be applied  \cite{crassidis2011optimal}.


\subsection{Linear Kalman Filter}
As aforementioned, the equations of the \gls{lkf} that are computed iteratively can be be split into two steps: The prediction and the correction. The prediction step performs a one-step-ahead prediction for the current state $\hat{\boldsymbol{x}}_{k}$ and the current error covariance matrix $\hat{\boldsymbol{P}}_{k}$, using the previous state $\boldsymbol{x}_{k-1}$, the previous error covariance matrix $\boldsymbol{P}_{k-1}$, the current control input $\boldsymbol{u}_{k}$ and three constant matrices \cite{kelly19943d}:

\begin{equation}
\hat{\boldsymbol{x}}_{k} = \boldsymbol{F} \boldsymbol{x}_{k-1} + \boldsymbol{G} \boldsymbol{u}_{k}
\label{eq:lkf_prediction_1}
\end{equation}
\begin{equation}
\hat{\boldsymbol{P}}_{k} = \boldsymbol{F} \boldsymbol{P}_{k-1} \boldsymbol{F}^T + \boldsymbol{Q} \\[1.25em]
\label{eq:lkf_prediction_2}
\end{equation}

$\boldsymbol{F}$, $\boldsymbol{G}$ and $\boldsymbol{Q}$ are the three constant matrices, representing the state transition model, the control input model and the covariance of the process noise respectively.

The correction step of the \gls{lkf} consists of the following equations \cite{kelly19943d}:

\begin{equation}
\boldsymbol{y}_{k} = \boldsymbol{z}_{k} - \boldsymbol{H} \hat{\boldsymbol{x}}_{k}
\label{eq:lkf_correction_1}
\end{equation}
\begin{equation}
\boldsymbol{S}_{k} = \boldsymbol{H} \hat{\boldsymbol{P}}_{k} \boldsymbol{H}^T + \boldsymbol{R}
\label{eq:lkf_correction_2}
\end{equation}
\begin{equation}
\boldsymbol{K}_{k} = \hat{\boldsymbol{P}}_{k} \boldsymbol{H}^T \boldsymbol{S}_{k}^{-1}
\label{eq:lkf_correction_3}
\end{equation}
\begin{equation}
\boldsymbol{x}_{k} = \hat{\boldsymbol{x}}_{k} + \boldsymbol{K}_{k} \boldsymbol{y}_{k}
\label{eq:lkf_correction_4}
\end{equation}
\begin{equation}
\boldsymbol{P}_{k} = (\boldsymbol{I} - \boldsymbol{K}_{k} \boldsymbol{H}) \hat{\boldsymbol{P}}_{k} \\[1.25em]
\label{eq:lkf_correction_5}
\end{equation}

Here, another three constant matrices, the observation model $\boldsymbol{H}$, the covariance of the measurement noise $\boldsymbol{R}$ and the identity matrix $\boldsymbol{I}$, and the current measurement $\boldsymbol{z}_k$ are introduced. In \autoref{eq:lkf_correction_1}, the innovation $\boldsymbol{y}_k$ is computed, which is the difference between the measurement and the current estimate. Therefore, the observation model is required, which maps the estimation to the measurement space. Next, \autoref{eq:lkf_correction_2} computes the predicted measurements noise covariance matrix $\boldsymbol{S}_k$, which is then used in \autoref{eq:lkf_correction_3} to compute the Kalman gain $\boldsymbol{K}_k$. The Kalman gain can be thought of as a blending value within the range $[0.0, 1.0]$ that decides how much of the innovation is considered in the final correction equations \autoref{eq:lkf_correction_4} and \autoref{eq:lkf_correction_5}, where the state and the error covariance matrix are corrected. If $\boldsymbol{K}_k= 0$, there is no correction. If $\boldsymbol{K}_k= 1$ the state is corrected with all the innovation \cite{welch1995introduction}.

Both steps, the prediction step and the correction step, are part of the main loop of the \gls{lkf} algorithm. Before the \gls{lkf} can be deployed, initial estimates for the state $\boldsymbol{x}_0$ and for the error covariance matrix $\boldsymbol{P}_0$ must be defined \cite{welch1995introduction}. \autoref{fig:kf} depicts the principle flow of a \gls{kf} which also represents the flow of the \gls{lkf}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{images/kalman_filter_flow.pdf}
\caption[Principle flow of a Kalman filter]{\textbf{Principle flow of a \gls{kf}.} A \gls{kf} is initialized with an initial estimate of the state vector $\boldsymbol{x}$ and the error covariance matrix $\boldsymbol{P}$. Within the loop $\boldsymbol{x}$ and $\boldsymbol{P}$ of the next time-discrete step $k$ is predicted with the influence of the control input $\boldsymbol{u}$ and if a measurement $\boldsymbol{z}$ for this time-discrete step is available, $\boldsymbol{x}$ and $\boldsymbol{P}$ are also corrected.}
\label{fig:kf}
\end{figure}

It is notable, that with each prediction, the uncertainty about the state increases as the error covariance matrix $\boldsymbol{P}$ accumulates due to the process noise $\boldsymbol{Q}$. With each correction, in turn, the uncertainty about the state decreases because the error covariance matrix $\boldsymbol{P}$ is reduced by the Kalman gain $\boldsymbol{K} \in [0..1]$. Therefore, the more measurements are available, the smaller the error covariance matrix $\boldsymbol{P}$ can become \cite{zhang2011evaluation}.

Furthermore, for a \gls{kf} to filter properly, $\boldsymbol{Q}$ and $\boldsymbol{R}$ must be well defined, where higher values in $\boldsymbol{Q}$ imply greater uncertainty in the system's dynamics, which can be interpreted as a level of distrust or uncertainty in the accuracy of the system's model. Accordingly, higher values in $\boldsymbol{R}$ indicates greater uncertainty in the measurements obtained, which again can be interpreted as a level of distrust or uncertainty in the accuracy of the measurements \cite{saha2013robustness}.


\subsection{Extended Kalman Filter}
The \gls{ekf} is an extension to the principals of the \gls{kf}. It can be applied to non-linear systems where the non-linear state transition model and the non-linear observation model are linearized using first-order Taylor series expansion. These linearizations introduce errors, particularly when the system is highly non-linear. There exist higher-order \gls{ekf}s, where more terms of the Taylor series expansions are retained for the linear approximation of the models. However, higher-order \gls{ekf}s tend to only provide performance benefits when the measurement noise is small and increase the computation demand tremendously. Furthermore, since the \gls{ekf} relays on Taylor series, the state transition and the observation models must be differentiable functions. The linearizations using the Taylor series expansion are used for predictive parts of the \gls{ekf}. Besides these linearizations, the \gls{ekf} requires further linearizations for the state error covariance updates. Therefore, the Jacobian \cite{gale1965jacobian} of the non-linear state transition model and the non-linear observation model must be computed \cite{einicke1999robust}, \cite{crassidis2011optimal}.

The equations for the prediction step and the correction step of the \gls{ekf} are very similar to those of the \gls{lkf}. For the prediction step, the following equations hold \cite{crassidis2011optimal}:

\begin{equation}
\hat{\boldsymbol{x}}_k= f(\boldsymbol{x}_{k-1}, \boldsymbol{u}_k)
\label{eq:ekf_prediction_1}
\end{equation}
\begin{equation}
\hat{\boldsymbol{P}}_k= \boldsymbol{F}(\boldsymbol{x}_{k-1}, \boldsymbol{u}_k) \boldsymbol{P}_{k-1} \boldsymbol{F}^T(\boldsymbol{x}_{k-1}, \boldsymbol{u}_k) + \boldsymbol{Q} \\[1.25em]
\label{eq:ekf_prediction_2}
\end{equation}

Where $f$ is the linearized non-linear state transition model and $\boldsymbol{F}$ is the Jacobian of $f$.

Similarly, the equations of the correction step are adjusted for the linearizations \cite{crassidis2011optimal}, \cite{kelly19943d}:

\begin{equation}
\boldsymbol{y}_k= \boldsymbol{z}_k - h(\hat{\boldsymbol{x}}_k)
\label{eq:ekf_correction_1}
\end{equation}
\begin{equation}
\boldsymbol{S}_k= \boldsymbol{H}(\hat{\boldsymbol{x}}_k) \hat{\boldsymbol{P}}_k\boldsymbol{H}^T(\hat{\boldsymbol{x}}_k) + \boldsymbol{R}
\label{eq:ekf_correction_2}
\end{equation}
\begin{equation}
\boldsymbol{K}_k= \hat{\boldsymbol{P}}_k\boldsymbol{H}^T(\hat{\boldsymbol{x}}_k) \boldsymbol{S}_k^{-1}
\label{eq:ekf_correction_3}
\end{equation}
\begin{equation}
\boldsymbol{x}_k= \hat{\boldsymbol{x}}_k+ \boldsymbol{K}_k\boldsymbol{y}_k
\label{eq:ekf_correction_4}
\end{equation}
\begin{equation}
\boldsymbol{P}_k= \big(\boldsymbol{I} - \boldsymbol{K}_t\boldsymbol{H}(\hat{\boldsymbol{x}}_k)\big)\hat{\boldsymbol{P}}_k\\[1.25em]
\label{eq:ekf_correction_5}
\end{equation}

Here, $h$ is the linearized non-linear observation model and $\boldsymbol{H}$ is the Jacobian of $h$. The Jacobian of the state transition model $\boldsymbol{F}$ and the Jacobian of the observation model $\boldsymbol{H}$ are defined as presented from \cite{crassidis2011optimal}:

\begin{equation}
\boldsymbol{F}(\boldsymbol{x}_{k-1}, \boldsymbol{u}_k) = \frac{\partial f(\boldsymbol{x}_{k-1}, \boldsymbol{u}_k)}{\partial \boldsymbol{x}}
\label{eq:ekf_jacobian_f}
\end{equation}
\begin{equation}
\boldsymbol{H}(\hat{\boldsymbol{x}}_k) = \frac{\partial h(\hat{\boldsymbol{x}}_k)}{\partial \hat{\boldsymbol{x}}} \\[1.25em]
\label{eq:ekf_jacobian_h}
\end{equation}


\paragraph{Extended Kalman Filter for Rotational and Translational Motion Estimations}\label{sec:ekf_state}
When designing an \gls{ekf} or another \gls{kf} for a system, firstly, the variables of the state vector must be defined. For this example, the state vector $\boldsymbol{x}$ is a 13-component tuple that includes the orientation (as quaternions) $\boldsymbol{q}$, the position $\boldsymbol{s}$, the angular velocities $\boldsymbol\omega$ and the translational velocities $\boldsymbol{v}$:

\begin{equation}
\begin{split}
\boldsymbol{x} &= {[\boldsymbol{q}, \boldsymbol{s}, \boldsymbol\omega, \boldsymbol{v}]}^T \\
&= {[q_{w}, q_{x}, q_{y}, q_{z}, s_x, s_y, s_z, \omega_x, \omega_y, \omega_z, v_x, v_y, v_z]}^T \\[1.25em]
\end{split}
\label{eq:ekf_state_vector_expanded}
\end{equation}

Alternatively, these state features can be represented using dual quaternions (see \autoref{sec:dual_quaternions}), but require therefore a state vector of the size 16. A larger state vector yields higher computational demand, which is why the dual quaternion state approach is disregarded for the \gls{ekf} in this work.

Next, the constant models and matrices are to be derived. Assuming all acceleration terms to be equal to 0, using \autoref{eq:motion_linear_way} and \autoref{eq:motion_linear_velocity} for the translational motion, and \autoref{eq:quaternion_estimator_q} and \autoref{eq:quaternion_estimator_w} for the rotational motion, a state transition model with no control input $f(\boldsymbol{x})$ for the state vector $\boldsymbol{x}$ can be built:

\begin{equation}
\begin{split}
f(\boldsymbol{x}) &=
\begin{bmatrix}
1 & 0 & 0 & 0 & 0 & 0 & 0 & -\frac{\Delta t}{2} q_{x} & -\frac{\Delta t}{2} q_{y} & -\frac{\Delta t}{2} q_{z} & 0 & 0 & 0 \\[6pt]
0 & 1 & 0 & 0 & 0 & 0 & 0 &  \frac{\Delta t}{2} q_{w} &  \frac{\Delta t}{2} q_{z} & -\frac{\Delta t}{2} q_{y} & 0 & 0 & 0 \\[6pt]
0 & 0 & 1 & 0 & 0 & 0 & 0 & -\frac{\Delta t}{2} q_{z} &  \frac{\Delta t}{2} q_{w} &  \frac{\Delta t}{2} q_{x} & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 1 & 0 & 0 & 0 &  \frac{\Delta t}{2} q_{y} & -\frac{\Delta t}{2} q_{x} &  \frac{\Delta t}{2} q_{w} & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & \Delta t & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & \Delta t & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & \Delta t \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1
\end{bmatrix}
\begin{bmatrix}
q_{w} \\[6pt]
q_{x} \\[6pt]
q_{y} \\[6pt]
q_{z} \\[6pt]
s_x \\[6pt]
s_y \\[6pt]
s_z \\[6pt]
\omega_x \\[6pt]
\omega_y \\[6pt]
\omega_z \\[6pt]
v_x \\[6pt]
v_y \\[6pt]
v_z
\end{bmatrix} \\[1.25em]
\end{split}
\label{eq:ekf_state_transition_model_expanded_pre}
\end{equation}

Which yields:

\begin{equation}
\begin{split}
f(\boldsymbol{x}) &=
\begin{bmatrix}
q_{w} - \frac{\Delta t}{2} q_{x} \omega_x - \frac{\Delta t}{2} q_{y} \omega_y - \frac{\Delta t}{2} q_{z} \omega_z \\[6pt]
q_{x} + \frac{\Delta t}{2} q_{w} \omega_x + \frac{\Delta t}{2} q_{z} \omega_y - \frac{\Delta t}{2} q_{y} \omega_z \\[6pt]
q_{y} - \frac{\Delta t}{2} q_{z} \omega_x + \frac{\Delta t}{2} q_{w} \omega_y + \frac{\Delta t}{2} q_{x} \omega_z \\[6pt]
q_{z} + \frac{\Delta t}{2} q_{y} \omega_x - \frac{\Delta t}{2} q_{x} \omega_y + \frac{\Delta t}{2} q_{w} \omega_z \\[6pt]
s_x + \Delta t v_x \\[6pt]
s_y + \Delta t v_y \\[6pt]
s_z + \Delta t v_z \\[6pt]
\omega_x \\[6pt]
\omega_y \\[6pt]
\omega_z \\[6pt]
v_x \\[6pt]
v_y \\[6pt]
v_z
\end{bmatrix} \\[1.25em]
\end{split}
\label{eq:ekf_state_transition_model_expanded}
\end{equation}

According to \autoref{eq:ekf_jacobian_f}, the Jacobian of the state transition model $\boldsymbol{F}(\boldsymbol{x})$ can be computed as follows:

\begin{equation}
\begin{aligned}
\boldsymbol{F}(\boldsymbol{x}) =
\bigg[\dfrac{\partial f(\boldsymbol{x})}{\partial q_{w}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial q_{x}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial q_{y}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial q_{z}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial s_{x}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial s_{y}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial s_{z}} &\\[2pt]
\dfrac{\partial f(\boldsymbol{x})}{\partial \omega_x} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial \omega_y} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial \omega_z} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial v_{x}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial v_{y}} \hspace{8pt}
\dfrac{\partial f(\boldsymbol{x})}{\partial v_{z}} &\bigg]
\end{aligned} \\[1.25em]
\label{eq:ekf_state_transition_jacobian_expanded_raw}
\end{equation}

Yielding the state transition model:

\begin{equation}
\begin{split}
&\boldsymbol{F}(\boldsymbol{x}) =\\[6pt]
&\begin{bmatrix}
1                           & -\frac{\Delta t}{2} \omega_x & -\frac{\Delta t}{2} \omega_y & -\frac{\Delta t}{2} \omega_z & 0 & 0 & 0 & -\frac{\Delta t}{2} q_{x} & -\frac{\Delta t}{2} q_{y} & -\frac{\Delta t}{2} q_{z} & 0 & 0 & 0 \\[6pt]
\frac{\Delta t}{2} \omega_x &  1                           & -\frac{\Delta t}{2} \omega_z &  \frac{\Delta t}{2} \omega_y & 0 & 0 & 0 &  \frac{\Delta t}{2} q_{w} &  \frac{\Delta t}{2} q_{z} & -\frac{\Delta t}{2} q_{y} & 0 & 0 & 0 \\[6pt]
\frac{\Delta t}{2} \omega_y &  \frac{\Delta t}{2} \omega_z &  1                           & -\frac{\Delta t}{2} \omega_x & 0 & 0 & 0 & -\frac{\Delta t}{2} q_{z} &  \frac{\Delta t}{2} q_{w} &  \frac{\Delta t}{2} q_{x} & 0 & 0 & 0 \\[6pt]
\frac{\Delta t}{2} \omega_z & -\frac{\Delta t}{2} \omega_y &  \frac{\Delta t}{2} \omega_x &  1                           & 0 & 0 & 0 &  \frac{\Delta t}{2} q_{y} & -\frac{\Delta t}{2} q_{x} &  \frac{\Delta t}{2} q_{w} & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & \Delta t &        0 &        0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 &        0 & \Delta t &        0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 &        0 &        0 & \Delta t \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\[6pt]
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1
\end{bmatrix} \\[1.25em]
\end{split}
\label{eq:ekf_state_transition_jacobian_expanded}
\end{equation}

The observation model $h(\boldsymbol{x})$ maps from the estimation space to the measurement space. Assuming to have only orientations and positions as measurements, the observation model $h(\boldsymbol{x})$ can be defined as:

\begin{equation}
h(\boldsymbol{x}) =
\begin{bmatrix}
1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0
\end{bmatrix}
\begin{bmatrix}
q_{w} \\
q_{x} \\
q_{y} \\
q_{z} \\
s_x \\
s_y \\
s_z \\
\omega_x \\
\omega_y \\
\omega_z \\
v_x \\
v_y \\
v_z
\end{bmatrix}
=
\begin{bmatrix}
q_{w} \\
q_{x} \\
q_{y} \\
q_{z} \\
v_x \\
v_y \\
v_z
\end{bmatrix} \\[1.25em]
\label{eq:ekf_observation_model_expanded}
\end{equation}

Similarly to the derivation of the Jacobian of the state transition model, the Jacobian of the observation model $\boldsymbol{H}(\boldsymbol{x})$ can be derived using \autoref{eq:ekf_jacobian_h}:

\begin{equation}
\begin{split}
\boldsymbol{H}(\boldsymbol{x}) &=
\begin{aligned}
\bigg[\dfrac{\partial h(\boldsymbol{x})}{\partial q_{w}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial q_{x}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial q_{y}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial q_{z}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial s_{x}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial s_{y}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial s_{z}} &\\[2pt]
\dfrac{\partial h(\boldsymbol{x})}{\partial \omega_x} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial \omega_y} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial \omega_z} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial v_{x}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial v_{y}} \hspace{8pt}
\dfrac{\partial h(\boldsymbol{x})}{\partial v_{z}} &\bigg]
\end{aligned} \\[8pt]
&=
\begin{bmatrix}
1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0
\end{bmatrix} \\[1.25em]
\end{split}
\label{eq:ekf_observation_jacobian_expanded}
\end{equation}

Under the assumption, that the noises of the features of the state are not correlated and thus off-diagonal entries are 0, the covariance of the process noise $\boldsymbol{Q}$ can be modelled in two ways \cite{formentin2014insight},

\begin{equation}
\boldsymbol{Q} = \boldsymbol{I}_{13} \, \sigma_Q^{2} \\[1.25em]
\label{eq:ekf_process_noise_single_expanded}
\end{equation}

where $\sigma_Q$ is a scalar representing the standard deviation of the process noise, and

\begin{equation}
\boldsymbol{Q} = \boldsymbol{I}_{13} \, \boldsymbol\sigma_{Q,13}^{2} \\[1.25em]
\label{eq:ekf_process_noise_multiple_expanded}
\end{equation}

where $\boldsymbol\sigma_{Q,13}$ is a vector representing multiple standard deviations of the process noise providing a scalar for each entry of the state vector $\boldsymbol{x}$:

\begin{equation}
\begin{aligned}
\boldsymbol\sigma_{Q,13} = [\sigma_{Q_{q_w}}, \sigma_{Q_{q_x}}, \sigma_{Q_{q_y}}, \sigma_{Q_{q_z}}, \sigma_{Q_{s_x}}, \sigma_{Q_{s_y}}, \sigma_{Q_{s_z}},&\\[2pt]
\sigma_{Q_{\omega_x}}, \sigma_{Q_{\omega_y}}, \sigma_{Q_{\omega_z}}, \sigma_{Q_{v_x}}, \sigma_{Q_{v_y}}, \sigma_{Q_{v_z}}&]^{T}
\end{aligned} \\[1.25em]
\label{eq:ekf_process_noise_multiple_entries_expanded}
\end{equation}

For the covariance of the measurement noise $\boldsymbol{R}$, also two models can be applied \cite{formentin2014insight},

\begin{equation}
\boldsymbol{R} = \boldsymbol{I}_7 \, \sigma_R^{2} \\[1.25em]
\label{eq:ekf_observation_noise_single_expanded}
\end{equation}

where $\sigma_R$ is a scalar representing the standard deviation of the measurement noise, and

\begin{equation}
\boldsymbol{R} = \boldsymbol{I}_7 \, \boldsymbol\sigma_{R,7}^{2} \\[1.25em]
\label{eq:ekf_observation_noise_multiple_expanded}
\end{equation}

where $\boldsymbol\sigma_{R,7}$ is a vector representing multiple standard deviations of the measurement noise providing a scalar for each entry of the measurement vector $\boldsymbol{z}$:

\begin{equation}
\boldsymbol\sigma_{R,7} = [\sigma_{R_{q_w}}, \sigma_{R_{q_x}}, \sigma_{R_{q_y}}, \sigma_{R_{q_z}}, \sigma_{R_{s_x}}, \sigma_{R_{s_y}}, \sigma_{R_{s_z}}]^{T} \\[1.25em]
\label{eq:ekf_observation_noise_multiple_entries_expanded}
\end{equation}

The last to defined constant matrix is the identity matrix $\boldsymbol{I}$ of \autoref{eq:ekf_correction_5}. Since the state vector has a length of 13, the identity matrix of this equation must be:

\begin{equation}
\boldsymbol{I} = \boldsymbol{I}_{13} \\[1.25em]
\label{eq:ekf_identity_expanded}
\end{equation}

With the equations \autoref{eq:ekf_prediction_1} to \autoref{eq:ekf_correction_5} and the models \autoref{eq:ekf_state_vector_expanded} to \autoref{eq:ekf_identity_expanded}, an \gls{ekf} for rotational and translational motion can be implemented, having orientations (as quaternions) and positions as measurement input.


\subsection{Unscented Kalman Filter}
The \gls{ukf} \cite{wan2001unscented} is another \gls{kf} approach to tackle non-linearities. It uses the \gls{ut} \cite{julier2002scaled}, also known as the \textit{Sigma-Point Transform}, to propagate the state and covariance through the non-linear functions directly, without linearization. By selecting a set of carefully chosen sigma points (sample points) and passing them through the non-linear functions via the \gls{ut}, the \gls{ukf} captures the distribution of the state variables. This approach tends to be more accurate in highly non-linear scenarios but may be computationally more demanding compared to the linearization approach of the \gls{ekf}. Furthermore, due to the higher degree of freedom from the additional free parameters in the \gls{ut}, the \gls{ukf} can be better tuned for different grades of non-linearity \cite{wan2001unscented}, \cite{kandepu2008applying}.

The principle procedure of the \gls{ukf} can be described by the following steps \cite{wan2001unscented}:

\begin{enumerate}
    \item Filter initialization: Definition of the initial state estimate and covariance matrix.
    \item Sigma points generation: Computation of a set of sigma points, using the mean and covariance of the current state estimate. These sigma points approximate the distribution of the current state more accurate than a linearization.
    \item Weights assignment: Weights are assigned to each sigma point, considering both the mean and covariance of the state distribution. These weights influence the contribution of each sigma point to the updated state estimate.
    \item Sigma points transformation: Each sigma point is transformed through the non-linear function that describes the system dynamics. This step captures the effect of the non-linearities in the system.
    \item Transformed mean and covariance computation: Computation of the mean and covariance of the transformed sigma points. This involves summing the weighted transformed sigma points to compute the updated mean and covariance of the state.
    \item Incorporation of measurements: If measurements are available, the predicted measurements and the actual measurements are used to update the state estimate. This step involves computing the Kalman gain, the measurement residual, and adjusting the state estimate based on the measurement information.
    \item Final Gaussian distribution computation: Utilizing the transformed mean and covariance, a Gaussian distribution that represents the updated state estimate can be computed. This distribution provides an accurate representation of the system's state, especially in the presence of non-linearities.
\end{enumerate}

The mathematical model and deviations, and more details about the \gls{ukf} can be found in the literature \cite{wan2001unscented}.


\section{Artificial Neural Networks}\label{sec:ann}
In the realm of \gls{ml}, learning tasks can be divided into two main approaches \cite{bishop2006pattern}:
\begin{itemize}
    \item \textit{Reinforcement learning}: Learning via interactions with an environment to maximize a reward signal.
    \item \textit{Data-driven learning}: Learning from data and optional corresponding labels to find underlying patterns in it.
\end{itemize}

Data-driven learning can be subdivided further into:
\begin{itemize}
    \item \textit{Supervised learning}: Learning classification, or regression from labeled data with explicit input-output pairs.
    \item \textit{Unsupervised learning}: Learning patterns, structures, or relationships in data without labeled examples.
\end{itemize}

In all of the above-mentioned subdivisions, \glspl{ann} find application. An \gls{ann} is a \gls{ml} model that is built after the principles of biological neural networks of animal brains \cite{brahme2014comprehensive}. The basic idea behind \glspl{ann} is to mimic the behavior of interconnected neurons in biological systems to process information. Therefore, multiple \textit{layers} consisting of artificial \textit{neurons} can be built, which can transmit signals to each other. Through iterative adjustments of the \textit{weights} and \textit{biases} of the neurons, machine learning can be achieved \cite{yegnanarayana2009artificial}. The weights are adjustable parameters that determine the strength of the connections to other neurons, while the biases are additional parameters that enable fine-tuning and shifting of the \textit{activation function}'s output of a neuron. Activation functions (e.g. sigmoid, tanh, \gls{relu}, Leaky\gls{relu} \cite{xu2020reluplex}) are mathematical functions applied to the output of each neuron in a layer to introducing non-linearity to the network and thus allow for learning complex, non-linear, relationships in the data.

The concept of \glspl{ann} is mathematically approved via the \textit{Universal Approximation Theorem} \cite{hornik1989multilayer}, which states that a \gls{fnn} with a single layer containing a finite number of neurons can approximate any continuous function, given enough neurons in that single layer. The \textit{Deep Universal Approximation Theorem} \cite{lu2017expressive} extends this concept, stating that given a \gls{fnn} with infinite layers (infinite depth) and a large number of neurons per layer, it is theoretically possible to approximate any continuous function, showcasing the potential power of depth in neural networks for representing complex functions.

In the Universal Approximation Theorems, the \glspl{fnn} are mentioned, which are the simplest class of \glspl{ann}. In \glspl{fnn}, information moves in only one direction, forward, without any cycles or loops. If in addition, each neuron in one layer is connected to every neuron in the subsequent layer, the \gls{ann} can be referred to as \gls{fcnn} or as dense neural network. With every additional layer in an \gls{ann}, the depth of it is increased. Thus, \glspl{ann} consisting of many layers can be considered as \gls{dnn}, where all layers between the input layer and the output layer are called \textit{hidden layers}. Accordingly, the number of neurons within each hidden layer is often named as \textit{hidden size}. The term \textit{deep} can generally be prefixed to any \gls{ann} if it has multiple hidden layers. \autoref{fig:ann} presents a \gls{fcnn} with two hidden layers.

\begin{figure}[!ht]
\centering
\includegraphics[width=\textwidth]{images/artificial_neural_network.pdf}
\caption[A fully connected neural network with two hidden layers]{\textbf{A \gls{fcnn} with two hidden layers.} The presented \gls{fcnn} consists of four layers: The input layer (green), two hidden layers (blue) and an output layer (yellow). All neurons of each layer are connected to all neurons of the adjacent layers.}
\label{fig:ann}
\end{figure}

In supervised learning, which is fundamental for this work, the so-called \textit{backpropagation} \cite{hecht1992theory} is required for an \gls{ann} to learn from data: After feeding the data forward through the network (forward pass), a loss from the output of the network and the ground truth is computed, which is then propagated back through the network to adjust all the weights and biases of each neuron along the \textit{computational graph} (backward pass). The computational graph represents the flow of data and operations as a directed graph where nodes depict mathematical operations and edges signify data flow through the network's layers. Applying the chain rule to the computational graph, the backpropagation computes the gradients that minimize the difference between the predicted and the actual outputs most, adjusting them iteratively during training.

Within every iteration of the training, \textit{batches} of the given data are processed. To train one \textit{epoch}, which refers to a complete iteration over all batches, the data must be split into such batches with a set \textit{batch size}. The batch size defines the number of samples that are propagated through the network with each iteration within the epoch. There are many approaches for a batch size selection, three principle approaches are \cite{masters2018revisiting}:

\begin{itemize}
    \item \textit{Full Batch}: All samples are used at once, which requires a lot of memory and slows down the training. This brings a lack of stochasticity to escape local minima, less generalization and thus the potential of overfitting, and no option to parallelize the learning using \glspl{gpu}.
    \item \textit{Mini Batch}: A small batch size compared to the amount of samples is used, which yields fast training and the potential lack of data context. For this scenario, processing of the batches can be distributed on \glspl{gpu}.
    \item \textit{Stochastic Batch}: With a batch size equal to 1, the gradient changes its direction very often which can be inefficient, suffers from a lack of data context and introduces more noise into the updates. However, the training is highly parallelizable and thereby fast, bringing the ability to not stay in local minima due to the high change rate of gradient direction. This approach is also referred to as \gls{sgd} \cite{bottou2010large}.
\end{itemize}

The choice of the right batch size depends on the task and on the data given. Mostly, mini batches are utilized, which strike a balance between the precision of the full batch and the computational efficiency of stochastic batch \cite{smith2017don}. Optimal batch sizes for parallelization on GPUs align with powers of 2 (e.g., 16, 32, 64, etc.), leveraging the inherent structure of \glspl{gpu} cores, which are designed in powers of 2 \cite{masters2018revisiting}.

Before batching the data, the data must be split into three datasets, required for the three phases of an \gls{ann} training: The training phase, the validation phase and the testing phase \cite{basheer2000artificial}. The first two phases are repeated for every epoch in a sequence, the testing phase is applied once after all epochs of training and validation phases:

\begin{itemize}
\item \textit{Training Phase}: In the training phase, first, the labeled training data is fed forward through the network. With the difference (error) between the predicted outputs and the actual labels, and a loss function that defines a loss policy, the loss is computed. Based on this loss, the gradients of the loss with respect to all the tensors that are involved in the computation graph are computed via the backpropagation. These gradients are optimized by an optimization algorithm and then applied to update the models' parameters (weights and biases in an \gls{ann}). By repeating this procedure, the training loss is minimized.
\item \textit{Validation Phase}: After the training phase, the trained model is validated using the labeled validation data by feeding the data forward through the network and computing the validation loss. In this phase, only the forward pass is applied to monitor how well it generalizes to data that is unseen from the training phase. At the end of this phase, the validation losses of this iteration are compared to those of previous epochs to save the best model.
\item \textit{Testing Phase}: When the model is trained and validated using the training and validation data over all epochs, the best model according to the validation loss is evaluated on a separate set of completely unseen data, the test data. As in the validation phase, only the forward pass is applied in this phase. This evaluation measures the model's performance on new, unseen data, simulating how well it might perform in real-world scenarios. The application of this phase where the model is used to make estimates on new, unseen data, is also referred to as \textit{inference}.
\end{itemize}

In the description of the \gls{ann} training phases, the mentioned \textit{loss function} and \textit{optimization algorithm} are both policies that must be defined before starting the training. The loss function defines the metric to compute the loss (e.g. \gls{mse}). The optimization algorithm defines a policy (e.g. \gls{adam} \cite{kingma2014adam}) that is applied to the computed gradients for the computational graph in order to optimize the update of the model's parameters.

Ideally, during the model training, the validation loss is at some point converging as a local minimum is found. Therefore, it is notable that when trying to learn more than one variable from a dataset, the training should not be separated to train each variable isolated. Such separations yield different local minimas for each separate training instead of a common local minima. Hence, such separations may increase the convergence time tremendously \cite{bertsekas1998network}. The convergence time is relevant, since it implies not only costs in time, but electricity costs, too.

If the validation loss is not converging, \textit{hyperparameters} may be tuned \cite{probst2019tunability}. Hyperparameters in machine learning refer to configuration settings or factors that are set prior to the model training and remain constant throughout the training. These parameters control the learning process and the model architecture, and affect the behavior and performance of the learning algorithm. Examples include the \textit{learning rate} in the optimization algorithm, which defines the step size of the applied parameter update, the number of layers in the \gls{ann} or the width of the hidden layers, the hidden size. In addition, a \textit{learning rate scheduler} can be implemented that adjusts the learning rate during training at different stages to facilitate convergence and improve training dynamically. For instance, decreasing the learning rate as training progresses might help the model to converge to a better minimum more efficiently, as with a fixed, too big, learning rate, where the training may only reach the surrounding of a local minima instead of getting very close to it. An example for such a scheduler is the \gls{relrop} which reduces the learning rate on validation plateaus, i.e. when the validation is not decreasing for a defined number of epochs \cite{feurer2019hyperparameter}.

If the validation loss is not only not converging but increasing while the training loss is still decreasing, \textit{regularization techniques} may be implemented to avoid the overfitting present in this case. Regularization techniques involve e.g. the following three techniques \cite{scholkopf2002learning}:

\begin{itemize}
    \item \textit{Early Stopping}: Stopping the training when the validation loss continues increasing for some epochs, avoids unnecessary training yielding an overfitted model. If the model of the best validation loss is saved and eventually utilized, the early stopping is not necessary to escape overfitting, but saves computational costs.
    \item \textit{Dropout}: Dropout is a regularization technique to prevent the model from relying too heavily on specific neurons. Therefore, during each training iteration, a random fraction of defined size of neurons in a defined layer is temporarily removed from the network.
    \item \textit{Weight Decay}: Weight decay or, \textit{L2 penalty}, is another regularization technique that adds a penalty term to the loss function to discourage the model from fitting the noise in the training data. The penalty term is the L2 norm of the model's weights, scaled by the predefined hyperparameter, the weight decay penalty term.
\end{itemize}

For the case of not achieving any learning at all, the hyperparameters, the model architecture and the data may be considered. For an \gls{ann} model to learn something useful, a pattern must exist in the data - having no structure in the data, no structure can be learned \cite{jain2020overview}. Furthermore, the task must be clear in order to select a suitable \gls{ann} architecture. For interpolation tasks (e.g. mapping or classification), \glspl{dnn} and \glspl{cnn} may be suitable. For tasks of extrapolation, (e.g. forecasting), in turn, \glspl{rnn} are a better fit \cite{deng2014tutorial}.

The just mentioned architectures, \gls{cnn} and \gls{rnn}, have the following properties:
\begin{itemize}
    \item \Glspl{cnn} \cite{li2021survey} are a type of \gls{ann}, designed for processing structured grid-like data, like images, by applying convolutions in layers to extract hierarchical features and by pooling layers to reduce dimensionality, enabling effective pattern recognition.
    \item A \gls{rnn} \cite{medsker2001recurrent}, on the other hand, is an \gls{ann} architecture that processes sequential data by utilizing recurrent connections, allowing it to retain and use information from previous steps (as additional input) while processing the new input.
\end{itemize}

Since \glspl{rnn} are suffering from the exploding and vanishing gradients problem \cite{hochreiter1998vanishing}, which describes that when gradients are greater than 1 they may become extremely large over time and when gradients are less than 1 they may become very small over time, extensions of \glspl{rnn} are proposed: The \gls{lstm} \cite{sherstinsky2020fundamentals} and the \gls{gru} \cite{dey2017gate}. Both of these architectures employ gated mechanisms to selectively retain and utilize information over sequential data. \Glspl{lstm} have a more complex gating structure compared to \gls{gru}, while \glspl{gru} exhibit a simpler and more compact design \cite{shewalkar2019performance}.

There are plenty more very useful \gls{ann} architectures, (e.g. Transformer \cite{vaswani2017attention}), but as these are not relevant for this work, they are left out. For further reading about successful \gls{ann} based model variations, see the literature \cite{da2017artificial}.


\section{Robot Operating System-Based Astrobee Simulation Environment}
\Gls{ros} \cite{quigley2009ros} is an open-source robotic framework for the designing, creating, and managing of complex robotic systems. Besides libraries and tools, \gls{ros} offers a communication network that is based on \textit{nodes} and \textit{topics}:

\begin{itemize}
    \item \textit{Node}: Nodes are individual software processes that are designed to perform specific tasks, such as controlling a sensor or processing data. Nodes can communicate with each other by publishing or subscribing to topics.
    \item \textit{Topic}: Topics are named buses over which nodes exchange messages. Nodes can publish messages to a topic or subscribe to a topic to receive messages.
\end{itemize}

The modular concept of nodes and topics enable a selective execution of nodes and asynchronous communication between nodes. Furthermore, \gls{ros} is language agnostic, which means that the underlying communication features to talk between nodes do not rely on a language, but on a lower layer instead. Hence, the modular concept of nodes also allows to write a node in different programming languages such as Python or \CC\hspace{0pt}. However, since \CC\hspace{0pt} is faster in execution \cite{zehra2020comparative} than Python, it is recommended writing nodes in \CC\hspace{0pt} when possible. The only fixed instance in \gls{ros} is the \textit{\gls{ros} master} which acts as centralized coordinator for all nodes and the communication.

\autoref{fig:ros} depicts the communication between nodes via topics within the \gls{ros} system.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{images/ros_communication.pdf}
\caption[Communication between nodes via topics within the Robot Operating System]{\textbf{Communication between nodes via topics within \gls{ros}.} In \gls{ros}, the communication between nodes is performed via topics. Asynchronously, nodes operate, publish and subscribe to topics after registering at the \gls{ros} master.}
\label{fig:ros}
\end{figure}

Based on \gls{ros}, the \gls{nasa} has built the \gls{ars} \cite{fluckiger2018astrobee} in order to operate with so-called \textit{Astrobees} \cite{bualat2018astrobee}. Astrobees are free-flying robots developed by the \gls{nasa} to assist astronauts and perform various experiments on the \gls{iss}. The Astrobee robots have the shape of a symmetric cube and are equipped with various sensors, a manipulator and a propulsion systems that allows them to navigate in the microgravity environment of the \gls{iss}.

With a default equipment setup, excluding a manipulator, Astrobees exhibit approximately similar principle axes of rotation \cite{ruggiero2021robust}. As for rigid bodies rotation are about its center of mass, the rotations of the Astrobee can be assumed to be about the geographical center of its cube-shaped body. Thus, rotations of the Astrobee can be assumed to be stable for small time intervals (hours).

The \gls{ars} brings a simulation environment with a \gls{gui} where multiple Astrobees can be spawned, controlled and visualized on a virtual \gls{iss}. Tasks like:

\begin{itemize}
    \item Vision-based localization and mapping
    \item Autonomous navigation, obstacle avoidance, and path planning
    \item Grasping objects, deploying payloads, and interacting with the environment using a robotic arm
\end{itemize}

can be safely simulated with the \gls{ars} before deploying and testing algorithms on the real \gls{iss} with real Astrobees.

Since \gls{ros} allows to record so-called \textit{rosbags} that contain messages with timestamps from selected topics, data from Astrobee simulations can be recorded and replayed to repeat an identical simulation or to use the data offline for other purposes.

\autoref{fig:astrobees} shows two free-flying Astrobees, where the yellow Astrobee is active, and the blue Astrobee is inactive, representing the roles of a chaser and a target.

\clearpage
\begin{figure}[!ht]
\centering
\includegraphics[width=0.9\textwidth]{images/astrobees.pdf}
\caption[Two free-flying Astrobees]{\textbf{Two free-flying Astrobees.} The yellow Astrobee is observing the state of the inactive blue Astrobee, illustrating a free-flying scenario in space with the roles of a chaser and a target. Adaption of an image from the \gls{nasa}\protect\footnotemark.}
\label{fig:astrobees}
\end{figure}

\footnotetext{Website: \url{https://www.nasa.gov/}, date: 07/17/2023}

